Learned Lock-free Search Data Structures

Non-blocking search data structures offer scalability with a progress guarantee on high-performance multi-core architectures. In the recent past, "learned queries" have gained remarkable attention. It refers to predicting the rank of a key computed by machine learning models trained to infer the cumulative distribution function of an ordered dataset. A line of works exhibits the superiority of learned queries over classical query algorithms. Yet, to our knowledge, no existing non-blocking search data structure employs them. In this paper, we introduce \textbf{Kanva}, a framework for learned non-blocking search. Kanva has an intuitive yet non-trivial design: traverse down a shallow hierarchy of lightweight linear models to reach the "non-blocking bins," which are dynamic ordered search structures. The proposed approach significantly outperforms the current state-of-the-art -- non-blocking interpolation search trees and elimination (a,b) trees -- in many workload and data distributions. Kanva is provably linearizable.

==> Diagram/LLC_MISS.tex <==
\begin{figure}[]
\captionsetup[subfigure]{justification=centering}
\centering
  \includegraphics[width=0.8\linewidth]{Diagram/img.pdf}
  \subfloat[]{  \includegraphics[width=0.48\linewidth]{Diagram/Read Heavy LLC Misses.pdf}}
   \subfloat[]{ 
  \includegraphics[width=0.48\linewidth]{Diagram/Update Heavy LLC Miss.pdf}}
\caption{Last-Level Cache Misses (Lower is better) (a) LLC misses on Read Heavy Workload, (b) LLC misses on Update Heavy Workload}
\label{fig:LLCMISS}
\end{figure}

==> Diagram/verlist.tex <==
\begin{figure}
% \begin{minipage}[t]{.48\textwidth}
% \begin{minipage}{.40\textwidth}
    \centering
    \includegraphics[width=.80\linewidth]{Diagram/vers_list.pdf}
    \caption{Vesrion Linked List and Version Array}
    \label{fig:vers_list}
    % \end{minipage}
    % \begin{minipage}[t]{.48\textwidth}
   % \end{minipage} 
    % \end{minipage}
\end{figure}
\begin{figure}[]
% \begin{minipage}{0.48\textwidth}
% \begin{minipage}{.6\textwidth}
    
\captionsetup[subfigure]{justification=centering}
\centering
  \includegraphics[width=0.80\linewidth]{Diagram/legend_rs.png}
  % \vspace{-5mm}
  \subfloat[]{  \includegraphics[width=0.49\linewidth]{Diagram/Rangesearch_Readheavy.pdf}}
   \subfloat[]{ 
  \includegraphics[width=0.49\linewidth]{Diagram/Rangesearch_Updateheavy.pdf}}

% \label{fig:range_search}
% \end{minipage}

\caption{\scriptsize a) Throughput of read-heavy workload with Range Search b) Throughput of update-heavy workload with Range Search }
\label{fig:range_search}
% \end{minipage}

% \end{minipage}
\end{figure}

==> Sections/Background_and_Motivation.tex <==
%\subsection{Comparison-based Concurrent Indexes}
\textbf{B+Tree and variants} are classical indexes where each $e_i\in\mathcal{E}$ is based on comparison operations with $B$ data points, stored in ``fat'' nodes. Some of the lock-free designs are lock-free B$^+$-tree \cite{braginsky+:SPAA:2012}, Open BW-Tree~\cite{wang2018building}, and BZ-Tree \cite{arulraj2018bztree}. %used arrays for fat nodes and managed the updates in mapping tables. Experiments showed that \cite{wang2018building} handled real-time data with good performance. Arulraj et al.~\cite{arulraj2018bztree} proposed another tree name BZ-Tree using multi-word compare and swap operation, outperforming Open BW-Tree by a good margin.

\textbf{$(a,b)$-Tree} derives from B$^+$-trees by relaxing the size of the fat nodes to vary between $a$ and $b$, whose lock-free implementation was introduced by \cite{TrevorBrown:PhDThesis}. Recently, Elimination (a,b) tree \cite{srivastava2022elimination}, a lock-based variant of ~\cite{TrevorBrown:PhDThesis}, which also uses elimination \cite{hendler2004scalable} of concurrent \insertADT and \remove operations with the same key, demonstrably outperformed several other classical concurrent indexes. 

%They perform a binary search at the nodes, wherein internal nodes are used for indexing, and data is stored in the array-based leaf nodes. The leaf nodes are updated under node-specific locks. 

Lock-free interpolation search tree \textbf{C-IST}~\cite{brown2020non} uses the interpolation search \cite{mehlhorn1993dynamic} to choose the child node for indexing. They are our nearest classical comparison-based index counterpart. Given a dataset of size $n$, the root node is of degree $\sqrt{n}$ covering the entire dataset and dividing it into $\sqrt{n}$ buckets. The child node of a bucket covering $\sqrt{n}$ keys will have $\sqrt[4]{n}$ degree. This rule-based division continues for $O(log~log~n)$ levels, ensuring expected amortized $O(log~log~n + p)$ steps for data structure operations on smooth key distributions, where $n$ is the dataset size at the invocation, and $p$ is the maximum number of threads. The data exists at leaf nodes. Interpolation search makes the indexing faster for favourable key distributions; however, rebalancing is costly in C-IST. The fat nodes are array-based and are reallocated and replaced using double-compare-single-swap (DCSS) for every update; however, the operations display good cache behaviour. By contrast, we never reallocate \mnd{s} and use only system native single-word \cas primitives.

\cite{wang2018building} and ~\cite{arulraj2018bztree} presented experimental results for range search queries. However, their implementations\textit{ are not \lble}. Others \cite{braginsky+:SPAA:2012}, \cite{TrevorBrown:PhDThesis}, \cite{srivastava2022elimination}, \cite{brown2020non} do not have any implementation of range search, though \cite{srivastava2022elimination} and \cite{brown2020non} mention that it can be implemented following \cite{brown2022pathcas}.

\ignore{\subsection{Learned Indexes}
\textbf{Recursive model index} (RMI) proposed by \cite{kraska2018case} uses a hierarchy $e_i\in\mathcal{E}$ of multi-layer perceptrons. A model predicts the model at the next level of hierarchy, thus providing a path to an approximate location of the query key in the sorted array of datasets at the leaf level. Models are chosen based on the key distribution, which also sets up a trade-off between the complexity of the model hierarchy and the prediction accuracy. The models are trained level by level, starting from the lowest one. RMI does not allow updates in the dataset. While the model hierarchy training in RMI requires accessing the dataset multiple times, \textbf{PGM-index}~\cite{ferragina2020pgm}, \textbf{FITing-tree}~\cite{galakatos2019fiting} and \textbf{Radix-Spline}~\cite{kipf2020radixspline} fit models in a single pass over the data with a fixed error bound, which reduced the index building cost. These schemes, in static cases, offer performance competitive with RMI.


ALEX~\cite{Alex} and dynamic PGM-Index~\cite{ferragina2020pgm} allow dynamic updates. The updates ingested in gapped arrays in ALEX or LSM-managed updates in PGM-Index naturally required retraining the models. In general, these sequential indexes implement range search as well. 
}
%\subsection{Learned Concurrent Indexes}
\textbf{XIndex} ~\cite{tang2020xindex} was the first learned index to support concurrent updates. Similar to classical B$^+$-trees, the dataset is stored in leaf nodes. The index uses the RMI \cite{kraska2018case}. Each leaf node contains an associated model for search. In addition, they contain buffers for ingesting updates. 
%A buffer is based on a Masstree~\cite{Masstree}, which is a cache-optimized fine-grained lock-based concurrent key-value store. 
 A query in a leaf node has to explore both the data and the buffer whereof searching in the buffer uses a comparison-based scheme. It uses background threads to merge the data and the buffer under barriers to maintain consistency, which blocks the update operation in the buffer. %If the existing model in the leaf node is not able to approximate keys on merging, the node is split. The compaction process runs in the background periodically without knowing the real-time status of the buffer. This periodic run in the background may make buffer size large and decrease the search speed by 3x~\cite{li2021finedex}. %Another key drawback is that data in leaf nodes are not fully sorted as stored in the buffer and model-managed data array; it causes a query to search in both the data array and buffer.


\textbf{\fdex}~\cite{li2021finedex}, which \kan builds on, addressed the drawbacks of XIndex. Firstly, in the leaf nodes, they used "bins" as in \kan, that enabled both cache-optimized read and lock-based concurrent updates, scrapping the need to explore the data array and buffer separately. %When a bin is full, it is converted to a data array, and its associated model is obtained by training on the local data, unlike retraining the entire RMI \cite{tang2020xindex}. 
They used a heuristic approach~\cite{xie2014maximum} to train the linear models with fixed error bound. 
%Initially, \fdex has a single hierarchy level with the root node containing $n$ keys and $n+1$ bin-pointers. As the new keys are inserted, bins are populated and converted to the data array with associated models and bin-pointers for the next level. This design allows containing data in internal nodes, thereby accelerating the lookups. Though it is an unbalanced index, the hierarchy is shallow for uniform key distributions. 
\fdex outperformed XIndex across the workloads and data distributions. As mentioned in Section \ref{sec:intro}, both \cite{tang2020xindex} and \cite{li2021finedex} support only non-\lble range search. 
\ignore{
\subsection{Review Summary}
The above algorithms and their implementations provide the following insights about the data nodes and indexes:
\begin{itemize}[noitemsep, topsep=0.2pt, leftmargin=*, nosep, nolistsep]
\item Cache locality optimization requires array-based fat nodes.
\item Reallocation of fat nodes is costly at every update. Moreover, the cost increases with the size of such nodes. However, for a lock-free implementation, reallocation of nodes becomes unavoidable in practice. Thus, we must aim to optimize the size of updatable nodes.
\item The model-equipped data arrays give better look-up performance only after the size is good enough for classical methods such as binary search to become relatively costly. Therefore, the leaf nodes should not contain too few keys.
\item The single-pass model training schemes, e.g. PLA in \cite{ferragina2020pgm}, do better than multi-pass training methods, e.g. RMI \cite{kraska2018case}. 
\item An initial shallower hierarchy is preferable to rebalancing approaches in a concurrent setting.
\end{itemize}

Drawing lessons from these insights, we describe the proposed lock-free learned index Kanva in the next section. Table \ref{Table:scalability} summarizes the concurrent and learned indexes. 


\myparagraph{Kanva}We propose Kanva, a first learned lock-free search tree-like structure that outperforms all the existing data structures with significant margins. Kanva uses a lock-free data structure at bins for new data to be inserted and trains the machine learning model to predict the child's position at the internal node. Internal nodes contain data and is indexed by linear models. Kanva is an unbalanced search tree and doesn't have to put any effort into balancing it, making it faster than its counterparts. Due to its fat internal nodes, there is much less contention, and the tree's height also doesn't grow much compared to the conventional tree. Table \ref{Table:scalability} shows the scalability of existing Learned-Index schemes. One can see that Kanva is the first scheme which supports linearizable Lock-Free concurrent updates with the help of a lock-free data structure in Bin.
}




==> Sections/Kanva_Design.tex <==
\subsection{Layout and Operations basics}

Structurally, \kan capitalizes on \fdex \cite{li2021finedex} to implement a \lble lock-free dynamic key-value store. \kan implements an ADT that we presented in the last section. Our approach for \lble range search requires pairing the values with their update timestamps drawing from \cite{wei2021constant}. For this purpose, we associate a list of objects packing a value and its corresponding update timestamp to a key. We refer to this object as \textit{\vval} or versioned-value. The design and evolution of \kan is shown in Figure \ref{fig:kanva-structure}. 


\textbf{Models:} We use \textbf{linear regression models} in \kan nodes to approximate the ranks of the keys as \[rank=a\times key + b + \epsilon.\] We apply a simple lock-free linear model fitting approach as described in Section \ref{sec:lfmodel}. Given a dataset as a sorted array of keys, models essentially approximate the CDF of key segments of the dataset. Thus, a set of models approximate the CDF of the dataset in a \textit{piecewise linear} fashion. A model is represented as a packet of parameters $\{a,b,\epsilon\}$.

\textbf{Hierarchical structure} of \kan as shown in Figure \ref{fig:kanva-structure}(a) is shallow and unbalanced. It comprises \textit{{internal nodes}} and \textit{{Bins}}. Both internal nodes and bins contain multiple key-value pairs and are updatable. 

\textbf{Internal nodes} consist of a sorted array of keys and an array of \vval pointers, see Figure \ref{fig:kanva-structure}(b). An internal node \textit{other than the root} is equipped with a single model. Internal nodes are also updatable: inserting a key-value pair with a new value updates the latest \vval object associated with the key, and a deleted key can be re-inserted with a new associated value. Each internal node other than the root is roughly equal in size, which is determined by the size threshold of a bin, which we specify below. An internal node containing $m$ keys has $m+1$ pointers to bins associated with it following the order of the keys. The bin pointers are $null$ until a key-value pair is stored.


\ignore{wiFor the  Unlike \fdex \cite{li2021finedex}, we apply a single pass over data to build the models and compute the error hyperparameter $\epsilon$. %We apply exponential search after estimating the approximate rank of a key for model enabled traversal.
 This approach is beneficial in a lock-free concurrent setting with dynamic updates also in the internal nodes.  
}
\textbf{Bins} of \kan ingest the insertion and deletion of key-value pairs. A bin is structurally different from an external node of a classic B$+$ tree. Therefore, we named them so. We initialize a bin as a sorted linked list called a \textbf{one-level bin}. As the number of key-value pairs in a one-level bin reaches its size threshold, it is replaced with a \textbf{two-level bin}. A two-level bin has an array for indexing and multiple one-level bin pointers, which can further store key-value pairs. As the number of keys in a two-level bin reaches its size threshold, it is replaced with an internal node containing its key-value pairs. The lifecycle of a bin is shown in Figure \ref{fig:kanva-structure}(d). %Searching for a key in a bin uses an ordered traversal.

\textbf{The root} of \kan is a unique internal node that contains the entire dataset at initialization; see Figure \ref{fig:kanva-structure}(c). It includes an array of models for a piecewise linear fitting to the entirety of the initially given dataset. Using a model fitting scheme described in Section \ref{sec:lfmodel}, we obtain key segments with an identical error-bound $\epsilon$ for linear regression models as mentioned above. %Thereby each element of the array \texttt{model[]} consists of one end-point of the corresponding segment and the slope of the linear model fitted to the same. 
Initially, $n+1$ bin pointers are available in the root to ingest the updates, where $n$ is the size of the initially given dataset. 

\myparagraph{Traversals} in \kan are powered by the ML models. With multiple key segments in the root, we start by searching a query key over the set of endpoints, often applying a binary search. Having searched the appropriate segment, we search the key in the segment enabled by its associated model. Thus, the approximate location of the key is fixed. After that, a binary search in a bounded vicinity, determined by the regression error $\epsilon$, is performed to find the key's exact (possible) location. We perform an exponential search in an internal node other than the root to find the precise location. Exponential search does not require computing $\epsilon$, which is beneficial in a lock-free setting, as we describe in Section \ref{sec:lfmodel}. %As the internal nodes also store key-value pairs, many operations terminate at them. 
An operation only travels to the next level if the query key is not found at an internal node. Thus, a shallow hierarchy substantially reduces the lookup cost in \kan. A linear search is performed in a one-level bin, whereas, in a two-level bin, a linear search follows a binary search to determine the appropriate one-level bin. %The steps to perform a search in the bins is encapsulated by the method $searchBin$ at line \ref{search:srch_bin}. Clearly, there is a single path of traversal for each operation to reach its destination starting from the root.

 


\subsection{Data types}
\input{Sections/app}

The objects to implement \kan are described in Algorithm \ref{fig::Model}.  
Both internal nodes and bins in \kan are instances of class \nd. An internal node instantiates the class \mnd (Modelled Node). A model is represented by a set of parameters as implemented by the class \model. An \mnd object encapsulates a \model array \texttt{models[]} fitted to the keys that it contains. The associated list of \vval objects is linked by their head pointers stored in the array \texttt{versions}. 

The class \bin maintains its size threshold and a boolean to indicate if it is a two-level bin. A \bin class is further inherited by the classes \tbin and \obin of which instances implement two-level bins and one-level bins, respectively. The keys and associated links to \vval objects are encapsulated by class \knd. The \vval objects instantiate the class \vval. 

An instance of \kan contains an atomic integer \texttt{Timestamp} that helps in versioning the updates to enable \lble range search as we discuss in Section \ref{sec:rangesearch}.

\subsection{Lock-free \insertADT, \remove, and \search}
\textbf{\seek} method implements traversals in \kan as described above, which every operation calls at the invocation; see Algorithm \ref{alg:code-traverse}. \seek calls the method $searchInMNode$ to determine the index of the key array where the key could be potentially located. If the key is not located in the \mnd, $searchInMNode$ returns the index of the \texttt{children} array, where seek should be directed to following the sorted order. As a requirement, \seek returns a packet of \mnd, the index of a child pointer or the index of the key if located, and an enumeration -- $\{\found, \nfound, \maybe\}$ -- of the status of locating the key. 

%Along with an \mnd the potential key location is also returned. If the traversal terminates at an internal node without finding the key, it returns \nul.

\input{algorithm/code-traverse}



%Algorithm \ref{fig:code} presents a pseudo-code of \search, \insertADT and \remove operations in \kan. Each operation starts a traversal with searching for a key at the root node. 

% If the query key is found in the data array of an internal node, it returns the \texttt{node} and \texttt{ix} as the index of the key in the data array. If \texttt{node's} levelNode is either \texttt{null} or contains \texttt{Bin} pointer it returns node and ix as -1. 
%
%If the seek method returns an index other than -1, then we can return the value from the ix position of the node's data array. Otherwise, we check the child node in levelNode[ix] at line \ref{srch:levelnode}. If the child node is null, then we can simply return null as the key doesn't exist; otherwise, the node is a Bin, and it searches for the key in the Bin.

\input{algorithm/read1}

\myparagraph{\insertADT} is given in lines \ref{insert} to \ref{insert_end} in Algorithm \ref{fig:code}. %It inserts the key and value if it doesn't exist in the structure. 
It performs traversal at line \ref{ins:find_idx} to find the node where the insert can happen. If the key is found in an \mnd, in that case, it attempts to update the corresponding value using an atomic compare-and-swap (\cas) in the method \textsc{writeValue}, which repeatedly attempts to update the value until a \cas succeeds. 

%If the key exists in a modelled data array in a \nd, and the corresponding value is a tombstone, the value is updated at line \ref{insert:value}. 

If the key doesn't exist in an \mnd, the operation will try inserting it in an appropriate $Bin$. If the $Bin$ doesn't exist, a new $Bin$ is created at line \ref{newlevelbinstart} and atomically inserted using a \cas at line \ref{levelcas}. If the $CAS$ operation fails at line \ref{levelcas}, then some other thread must have added the $Bin$, and therefore the operation is retried. If the $Bin$ exists and has reached the threshold or is already undergoing transformation to a \mnd, it will engage in helping via method $\textsc{helpMakeModel}$ at lines \ref{ins:makemodel} or \ref{ins:makemodel1}. After any such possible help, insertion is attempted in a bin using method $insertBin$, whose result is returned finally.

\myparagraph{\remove} is given in lines \ref{del:start} to \ref{del:end}. \kan doesn't perform the physical deletion of a key. Instead, it marks the key as deleted by updating its value to \nul. In that way, a \remove operations works exactly like an \insertADT operation to update the corresponding value of a present key. If the key is not found it returns \fal. %Notice that, deletion does not 

%possibly located in a bin, its deletion resembles adding a tombstone at the key or returning  at line \ref{del:delbin}.


%\myparagraph{Model Creation}, as described in lines \ref{help_model}-\ref{helpmodel:end}, essentially collects all the keys from a \tbin to create a model and returns its corresponding key and value sets. Model creation is detailed in the next section. 


%If the Key is not present in the data array, then we search for the Key in its respective $Bin$ in $levelNode$. If the $Bin$ doesn't exist, then the Key to be deleted doesn't exist in the data structure. Otherwise, the key is deleted from the $Bin$. The deletion operation is essentially similar to that in the lock-free linked list of \cite{Harris:NBList:DISC:2001}.

\myparagraph{\search} operations, given in lines \ref{srch:start} to \ref{search:srch_bin} in Algorithm \ref{fig:code}, similarly starts with calling \texttt{Seek} in line \ref{srch:seek}. In case \seek returns \found or \maybe, and the fact that for the deleted keys, the corresponding values are \nul, it is straightforward for a \search operation to implement its ADT definition. If \seek returns \nfound, \search returns \nul.

\myparagraph{Helping} is performed in the method \textsc{helpMakeModel} as given in Algorithm \ref{alg:help}. Essentially, helping is required when a bin reaches its threshold. For both \obin and \tbin, we start with freezing its \knd{s}. For this purpose, we adopt the popular bit-stealing technique \cite{Harris:NBList:DISC:2001} to use one of the unused bits of their next pointers. On observing a frozen bin, $insertBin$ and $deleteBin$ operations result into indicating that a \insertADT and \remove operation need to engage in helping. Once an \obin is frozen, a \tbin replaces it appropriately. For a frozen \tbin, a key array is created of the keys collected from all its \obin{s}. After that, we perform a lock-free model training on this key array as described in Section \ref{sec:lfmodel} using the method \textsc{makeModel}. The created model and key array make a new \mnd; see line \ref{help:newmnode}.  



\input{algorithm/help_make_model.tex}

\ignore{
\subsection{Non-blocking Progress and Linearizability}

The update operations perform write using a single word atomic CAS. Whenever, a CAS fails, it either retries or helps. For example, two update operations at a key in a node, which is not a \bin may obstruct each other. In this case, one fails and retries its operation. On the other hand, if an update operation is obstructed by a frozen node in a \obin, it first helps the operation that would have triggered the freezing. The insert and remove operations in non-blocking linked-list of \cite{Harris:NBList:DISC:2001} carry their property from its basic design. The read operations do not either obstruct any operation or engage in helping. This establishes that at least one thread will complete its operation in a finite number of steps in a concurrent execution, proving the implementation lock-free.

The linearizability of ADT operations is proved by ordering them in an arbitrary concurrent execution by their linearization points (LPs). The LP of a successful update -- insert or delete -- operation at a node that is not a \bin happens at the successful atomic CAS. In case the update operation takes place in a \bin, it will be according to the LP of the same operation in the non-blocking linked-list of \cite{Harris:NBList:DISC:2001}. For an unsuccessful delete operation it will be at the invocation if the key was not present in the data structure or immediately after the concurrent delete operation that would have removed the key. The LP of an unsuccessful search operation is determined similar to an unsuccessful delete operation, whereas a successful search operation linearizes at the atomic read step where it first reads the query key in the data structure.      

The structure of a node of \kan is shown in Figure \ref{fig::Model}.  It contains arrays of keys, values, model\_or\_bin and Models. The array of models keeps all the linear models used to predict the position of the key in the sorted array, whereas array of model\_or\_bin keeps the entry of all the model\_or\_bin at lower level. A bin is a non-blocking data structure used to perform all the update operations. \kan provides the modularity where you can plug in any non-blocking data structure for the Bin, for high scalability. To achieve the high scalability we have designed a non-blocking \tbin.
	
Model and Bins are part of the basic structure of \kan, for linear prediction as well as the new updates, respectively.

The structure of a node of \kan is shown in Figure \ref{fig::Model}. A node of \kan contains arrays of keys, values, an array of Node$\ast$ called level\_bin and an array of Linear Models called models. The array of models keeps all the linear models used to predict the position of the key in the sorted array, whereas the level\_bin array keeps the pointers of all the models or bins at a lower level. Initially, a pointer at the level\_bin is Bin and replaced by a node once it has reached a threshold.
}


\ignore{
	\myparagraph{\tbin:} A non-blocking \tbin in \kan has a design similar to a B-Tree that can not expand beyond two levels. See Figure \ref{fig:Bin}. Initially, it has only one level as a linked list, which is replaced by a \tbin once its size reaches a threshold. In the \tbin, the first level is an array containing the keys and the pointers to the \cbin. The \cbin cotains non-blocking linked lists \cite{Harris:NBList:DISC:2001}. The \insertADT, \remove and \search operations take place in the \cbin whereas the array at the first level is used only for indexing. A \cbin is split into two, once it reaches the threshold. For splitting, it is \textit{frozen} by collecting all the elements and putting ``freezing markers'' in the node pointers of the linked list. Essentially, the freezing markers are the second least significant bit out of unused bits in the pointers. Once two new \cbin are created, the array at the first level is replaced atomically, with an array containing the newly created \cbin index and their pointers.
	
	While splitting a \cbin, if there is no space available in the array at the first level to accommodate a new \cbin, then the Bin is considered full. Once the Bin is full, it has to be entirely frozen before we retrain it to convert to a node. The procedure of freezing is the same as before -- we used the same unused bits of the next pointers of every linked-list-node. Once the Bin is frozen, all the elements from the Bin are collected to fit the models. Once the model is created, it replaces the current bin using a single word CAS operation. The lifecycle of a two-level can be seen in Figure \ref{fig:Lifecycle}.
}
\ignore{
	At the same time, Bins are used to achieve scalability with the help of its non-blocking concurrent data structure.
	
	They are maintained to avoid collision among the threads and provide high scalability in a non-blocking linearizable manner.
	
	To prevent conflicts, updates in the bins don't change the data array in the models, but
	
	
	The bins  the lookups easier with the data is kept sorted and don't need to search the delta-buffer before performing search operations in the model. %\spnote{I think it will be better to start with the explanation of the various data-structures used.}
	
	
	\kan introduces a new non-blocking approach for update operations and retraining the Bins to Model. Bins are a non-blocking data structure where all the new updates take place. Once the Bin is full it is retrained to a model and added to the next level. These operations take place concurrently without blocking other threads, leading to high scalability. Retraining of Bin is divided into four parts freezing, collection, training, and merging. In the freezing phase, once the Bin is Full, it will be frozen so that no more updates can take place to the Bin. Once the Bin is frozen, all the elements are collected from the Bin and then retrained to a new model. Once the new model is created, it will be added to the data structure atomically with the help of compare and swap operation. All the threads helps in retraining of Bin without blocking.
}


\ignore{
	In building the data structure, the root node contains the models, which helps in finding the key's position in the initialized sorted data array. A collection of $n+1$ $Bins$ $(B\_1, B\_2,..., B\_{n+1})$ are associated with $n$ keys similar to the child pointers in a classical B$^+$ tree node. A Bin is an ordered data structure that needs to support concurrent non-blocking linearizable ADT operations. The \insertADT, \remove and \search operations in bins also need to synchronize with model training in a non-blocking fashion once it is full. Notice that a \tbin only supports comparison-based traversal. Once a Bin is full, which is decided by a threshold, its data is collected, and a Linear Model is trained over the collected Keys
	
	
	
	\begin{figure}
		\centering
		\includegraphics[width = 1 \linewidth]{Diagram/design.pdf}
		\caption{\kan Design Structure}
		\label{fig:Kanva_Design}
	\end{figure}
	
	\ignore{
		\myparagraph{Transformation of a \bin:} starts with setting a special \textit{freezing} marker on the next pointers of each of its \obin nodes. In implementation, the freezing markers are essentially the second least significant bit out of unused bits in the pointers (the least significant bit is used by lock-free the linked-list operations). As soon as a concurrent modification -- \insertADT/\remove -- operation discovers any frozen pointer, it helps the operation that would have triggered the freezing. A frozen \obin node is immutable; however, unlike \fdex where the locks are at the granularity of bins, our fine-grained freezing approach allows better progress of concurrent operations.
	}
	%While splitting a leaf node, if there is no space available in the array items in the \tbin node to accommodate a new one-level node, then the Bin is considered full. Once the Bin is full, it has to be entirely frozen before we retrain it to convert to a node. The procedure of freezing is the same as before -- we used the same unused bits of the next pointers of every One\_Level\_Bin node. Once the Bin is frozen, all the elements from the Bin are collected to train a model. Once the model is created, a new Node is created and it replaces the current bin using a single-word CAS operation. The lifecycle of a two-level can be seen in Figure \ref{fig:Lifecycle}.
	
	
	
	%\kan supports all the basic index operations such as contains, delete and read. We will discuss most of these operations in detail in later sections.
	
	%The ADT operations in \kan use the hierarchy of ML models (hereafter referred to as models) to predict the key's position in the dataset, making it much faster than the conventional tree structure. 
	
	
	%If the $Bin$ is a $child\_bin$ and the size of the $child\_bin$ is less than the threshold, \insertADT operation tries to insert in the $child\_bin$; otherwise, if the size of the $child\_bin$ has reached the threshold it needs to be trained to create a linear model. To train a linear model, $child\_bin$ is frozen first as done by Braginsky and Petrank in \cite{braginsky+:SPAA:2012}. To freeze the linked list in the $child\_bin$ the second least significant bit of the next pointer is used to mark it frozen (cite harris) \cite{Harris:NBList:DISC:2001}. Once it is frozen, no more updates can occur in the $child\_bin$, and all the keys are collected for training. A new $Bin$ is created by having the pointer to the new $child\_node$ having a linear model trained with the keys collected from the $child\_bin$. $child_node$ also contains the array of data and values collected from the $child\_bin$. $Bin$ with the new $child\_node$ is replaced with the current $Bin$ using a single-word atomic $CAS$ operation at line \ref{ins:bin_cas}, and if the $CAS$ operation failed then some other thread must have successfully replaced this $Bin$ with a new $Bin$ having a $child\_node$ at line \ref{ins:bin_cas}. After performing the $CAS$ operation it will retry the \insertADT.  If the $level\_bin$ is a node, the operation recursively performs the \insertADT operation at the $child\_node$ of the $Bin$ at line \ref{ins:node}.  
	% \input{algorithm/Update}
	% \input{algorithm/insert}
	
	% \input{algorithm/insertanddelete}
	
}

%The value objects change temporally, and to support \lble range queries, which we describe in detail in Section \ref{sec:rangesearch}, timestamped values are stored in \texttt{VNode} objects. \texttt{vals[]} array. Thus, \kan implements a key-value store. Notice that every node in \kan contains a subset of the given dataset to build the index on. Therefore, for many data points, it is a much smaller traversal path for a query. A \nd also contains an array of pointers \texttt{levelNode[]} to nodes of type \bin{s} to ingest the updates. The size of the array \texttt{levelNode[]} is \textit{one more than that of} \texttt{keys[]} quite similar to a typical fat node in data structures such as B-trees, where a comparison with a key in a fat node decides the next node in the hierarchy. In addition, a node also contains an array of Version Node pointers (VNodes), which are used to support \lble \range queries.




%
%\begin{figure}[h!]
%	% \begin{minipage}{0.4\linewidth}
	%		\centering
	%		\includegraphics[width = 0.8 \linewidth]{Diagram/2-bin.pdf}
	%		\caption{Two-level Bin}
	%		\label{fig:Bin}
	%	% \end{minipage}
%\end{figure}

% \begin{figure}[h!]
	% 	% \begin{minipage}{0.59\linewidth}
		% 		\centering
		% 		\includegraphics[width = 0.95 \linewidth]{Diagram/Lifecylce.pdf}
		% 		\caption{Life Cycle of a Bin}
		% 		\label{fig:Lifecycle}
		% 	% \end{minipage}
	% \end{figure}
%\myparagraph{Bin:} An object of the class \bin ingests updates in a lock-free way. Initially, it gets instantiated as an object of subclass \obin (One-Level Bin). A \obin is a lock-free linked list, whose design draws from the well-known algorithm of Harris \cite{Harris:NBList:DISC:2001}. %The \insertADT, \remove and \search operations in a Bin actually takes place in a \obin. 
%A \bin object has a threshold on its size. As a \obin object reaches its threshold by \insertADT operations, it is replaced by an object of the subclass \tbin (Two-Level Bin), which has a design similar to a two levels B-Tree, see Figure \ref{fig:Bin}. %The design draws from that of bins in FINDex \cite{li2021finedex}, however it is fully lock-free. Unlike \cite{li2021finedex}, who use a lock for an entire two-level bin, thereby achieving a very limited concurrency, we allow lock-free updates to it as long as its threshold does not reach. 
%Essentially, in a \tbin, the first level is an array used for indexing the one-level bins at the lower levels. As the threshold of a \tbin reaches it is replaced with a node with models and the keys in all its \obin are shifted to the \texttt{keys[]} array of the node, and similarly the corresponding values. We often refer to such a node as \textit{a modelled node} (LNode). The life-cycle of a \bin has been shown in Figure \ref{fig:Lifecycle}. 
% \begin{figure}
	% 		\centering
	% 		\includegraphics[width = 0.95 \linewidth]{Diagram/Lifecylce.pdf}
	% 		\caption{Life Cycle of a Bin}
	% 		\label{fig:Lifecycle}
	% \end{figure}


==> Sections/abstract.tex <==
Lock-free concurrent data structures implemented on today's multicore computers offer throughput, scalability, and guarantees for the completion of operations. Recently, queries using machine learning models trained to predict the data distribution have gained remarkable attention. Yet, to our knowledge, no existing lock-free data structure employs them. This paper introduces a lock-free search structure that supports concurrent updates, membership, and range queries accelerated by a shallow hierarchy of lightweight machine learning models. The proposed approach significantly outperforms the current state-of-the-art in many workload and data distribution settings. Ours is the first provably linearizable learned lock-free concurrent range search index. 

==> algorithm/Delete.tex <==
\begin{algorithm}
\footnotesize
\caption{\texttt{\textbf{Delete}}(key)}
\label{Alg::delete}
$ix := models \rightarrow find\_idx(key)$\;
\If{keys[ix] = key}
{
    update the value of the key with a tombstone\;
    \label{delete:value}
    \texttt{\textbf{return}} true
}
\Else{
    \texttt{retry}: \;
    $current\_level\_bin :=  level\_bin[ix]$\;
    \If{$current\_level\_bin == null$}
    {
      return false
    }
    \ElseIf{$current\_level\_bin\rightarrow is\_node$}
    {
        \texttt{\textbf{return}} $current\_level\_bin \rightarrow child\_node \rightarrow Delete(key)$
    }
    \Else{
        $res = current\_level\_bin\rightarrow bin \rightarrow remove(key)$\;
        \If{$res == frozen$}{
        $new\_level\_bin$ := new Bin()\;
        $new\_level\_bin \rightarrow is\_node := true$\;
        $bin\_keys, bin\_vals := current\_level\_bin\rightarrow bin \rightarrow collect()$\;
       $new\_level\_bin \rightarrow child\_node := new Node(bin\_keys,bin\_vals)$\;
       $level\_bin[ix].\texttt{\textbf{CAS}}(current\_level\_bin, new\_level\_bin)$\\
       \texttt{\textbf{goto}} retry
        }
        \Else{return res}
    }
}
\end{algorithm}

==> algorithm/Update.tex <==
\begin{algorithm}
\caption{\texttt{\textbf{Insert}} (key, value)}
\label{Update}
\footnotesize

$ix := model \rightarrow find\_idx(key)$\;
\If{keys[ix] = key}
{
    update the value of the key\;
    \label{update:value}
    \texttt{\textbf{return}} true
}
\Else{
    \texttt{retry}: \;
    $current\_level\_bin :=  level\_bins[ix]$\;
    \If{$current\_level\_bin == null$}
    {
    %   $new\_level\_bin := level\_bins[ix]$\;
    %   \If{$new\_level\_bin = null$}{
       $new\_level\_bin := new model\_or\_bin()$\;
       \label{newlevelbinstart}
       $new\_level\_bin \rightarrow is\_model := false$\;
       $new\_level\_bin \rightarrow bin :=$ new Bin()\;
       \label{newlvwlbinend}
       $level\_bin[ix].\texttt{\textbf{CAS}}(current\_level\_bin, new\_level\_bin)$
       \label{levelcas}
       \texttt{\textbf{goto}} retry\;
       \label{updateretry1}
    %   }
    }
    \ElseIf{$current\_level\_bin\rightarrow is\_model$}
    {
        \texttt{\textbf{return}} $current\_level\_bin \rightarrow model \rightarrow insert(key, value)$
    }
    \Else{
        \If{$current\_level\_bin\rightarrow bin \rightarrow size \geq threshold$}{
        $new\_level\_bin := new model\_or\_bin()$\;
        $new\_level\_bin \rightarrow is\_model := true$\;
        $current\_level\_bin\rightarrow bin \rightarrow freeze()$\;
        $bin\_keys, bin\_vals := current\_level\_bin\rightarrow bin \rightarrow collect()$\;
       $new\_level\_bin \rightarrow model :=$ new model(keys,vals)\;
       $level\_bin[ix].\texttt{\textbf{CAS}}(current\_level\_bin, new\_level\_bin)$
       \texttt{\textbf{goto}} retry\;
        }
        \ElseIf{$current\_level\_bin\rightarrow bin \rightarrow insert(key,value)$}
        {
            \texttt{\textbf{return}} true
        }
        \Else{\texttt{\textbf{goto}} retry} 
    }
}
\end{algorithm}


==> algorithm/balance_leaf.tex <==
\begin{algorithm}[H]
\label{balanceleaf}
\caption{\texttt{balanceLeaf}(prevNode,\ prevIdx,\ currNode,\ currIdx)}
$\textup{Node* } newNode$\;
\uIf{$count \geq MAX$} 
{
    $newNode :=$ \texttt{splitLeaf}($prevNode,\ prevIdx,\ currNode,\ currIdx$)\;
    \label{alg8:line122}
}
\uElseIf{$count < MIN$}
{
    $newNode :=$ \texttt{merge}($prevNode,\ prevIdx,\ currNode,\ currIdx$)\;
    \label{alg8:line124}
}
\Else
{
    $newNode :=$ \texttt{createNewLeaf}($prevNode,\ prevIdx,\ currNode,\ currIdx$)\;
    \label{alg8:line126}
}
\textbf{return} $newNode$\;
\end{algorithm}

==> algorithm/balance_root.tex <==
\begin{algorithm}[H]
\label{balanceroot}
\caption{\texttt{balanceRoot}()}
$\textup{Node* } newNode$\;
\uIf{$isLeaf\ \&\&\ frozen$}
{
    \textbf{if} {$count \geq MAX$} \textbf{then} $newNode :=$ \texttt{splitRootLeaf}()\;
    \textbf{else} $newNode :=$ \texttt{createNewLeaf}()\;
}
\textbf{else if} {\textup{!}$\,isLeaf\ \&\&\ count \geq MAX$} \textbf{then} $newNode :=$ \texttt{splitRootInternal}()\;
\textbf{if} {\textup{!}$\,root$.\texttt{CAS}($\textit{\textit{\textbf{this}}},\  newNode$)} \textbf{then} \textup{\textbf{return}} \texttt{nullptr}\;
\textbf{else} \textbf{\textup{return}} $newNode$\;
\end{algorithm}

==> algorithm/borrow_helper.tex <==
\begin{figure}
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{}
\scriptsize
\algrestore{splitLeaf}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\Procedure{\textbf{mergeHelper}}{rightChild,\ rightIdx,\ leftChild,\ leftIdx,\ prev,\ pidx,\ curr}
\label{mergehelper}
% \caption{\texttt{mergeHelper}(rightChild,\ rightIdx,\ leftChild,\ leftIdx,\ prev,\ pidx,\ curr)}
\State{\textup{Node*} $newNode$}
\If{$rightChild \rightarrow count + leftChild \rightarrow count < MAX$}
% {
    \State{\textup{Node*} $newChild$}
    \If{$leftChild \rightarrow isLeaf$}
    % {
        \State{$newChild :=$ \texttt{new LeafNode()}}
        \State{$newChild \rightarrow next := rightChild \rightarrow next$}
    % }
    \Else
    % {
        \State{$newChild :=$ \texttt{new InternalNode()}}
    % }
    \EndIf
    \State{Merge $rightChild$ and $leftChild$ into $newChild$}
    \label{alg15:line185}
    \If{\textup{!}$\,leftChild \rightarrow newNext$.\texttt{\textup{CAS}}(\texttt{\textup{nullptr}}, $newChild$)}
    % {
        \label{alg15:line186}
        \State{$newChild := leftChild \rightarrow newNext$}
    % }
    \EndIf
    \State{$newNode :=$ \texttt{new InternalNode()}}
    \State{Copy every element in $curr$ into $newNode$ replacing pointers $leftChild$ and $rightChild$ with $newChild$}
    \label{alg15:line189}
% }
\Else
\State{$newNode :=$ \texttt{borrowHelper}($rightChild,$ $\ rightIdx,$ $\ leftChild,$ $\ leftIdx,$ $\ curr$)}
\EndIf
\If{$prev =$ \texttt{\textup{nullptr}}}
% {
    \If{$newNode \rightarrow count = 0$} 
    % {
        \State{$newNode := newChild$ (this occurs only when the left and right children are merged and newNode has only one child)}
    % }
    \EndIf
    \If{\textup{!}$\,root$.\textup{\texttt{CAS}}($curr, newNode$) }
    \State{ \textbf{return} \textup{\texttt{nullptr}}}
    \label{alg15:line194}
    \EndIf
% }
\ElsIf{\textup{!}$\,prev \rightarrow ptr[pidx]$.\texttt{CAS}($curr, newNode$)}
\State{\textbf{return} \textup{\texttt{nullptr}}}
\label{alg15:line195}
\EndIf

\State{\textbf{return} $newNode$}
\EndProcedure
\algstore{mergeHelper}
\end{algorithmic}
\caption{Pseudocode of mergeHelper}
\end{figure}
% \hrule
\begin{figure}
% \hrule
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\scriptsize
\algrestore{mergeHelper}
\Procedure{\textbf{borrowHelper}}{rightChild, rightIdx, leftChild, leftIdx, currNode}
\State{\textup{Node*} $newLeftChild$}
\State{\textup{Node*} $newRightChild$}
\If{$leftChild \rightarrow isLeaf$}
% {
    \State{$newLeftChild :=$ \texttt{new LeafNode()}}
    \State{$newRightChild :=$ \texttt{new LeafNode()}}
    \State{$newLeftChild \rightarrow next := newRightChild$}
% }
\Else
% {
    \State{$newLeftChild :=$ \texttt{new InternalNode()}}
    \State{$newRightChild :=$ \texttt{new InternalNode()}}
% }
\EndIf
\State{Copy every element in $leftChild$ and $rightChild$ into $newLeftChild$ and $newRightChild$ respectively}
\If{$leftChild \rightarrow count < MIN$}
% {
    \State{Move the first key in $newRightChild$ into the end of $newLeftChild$}
% }
\Else
\State{Move the last key in $newLeftChild$ into the beginning of $newRightChild$}
\EndIf
\If{\textup{!}$\,leftChild \rightarrow newNext$.\textup{\texttt{CAS}}(\textup{\texttt{nullptr}}, $newLeftChild$)}
% {
    \State{$newLeftChild := leftChild \rightarrow newNext$}
    \State{$newRightChild := rightChild \rightarrow next$}
% }
\EndIf
\State{\textup{Node*} $newNode =$ \texttt{new InternalNode()}}
\State{Copy every element in $currNode$ into $newNode$ replacing pointers $leftChild$ and $rightChild$ with $newLeftChild$ and $newRightChild$ respectively}
\State{\textbf{return} $newNode$}
\EndProcedure
\algstore{borrowhelper}
\end{algorithmic}
% \end{multicols}
\caption{Pseudocode of borrowHelper}
\end{figure}

==> algorithm/delete_leaf.tex <==
\begin{algorithm}[H]
\label{deletefromleaf}
\caption{\texttt{deleteFromLeaf}(key)}
\textbf{if} $frozen$ \textbf{then} \textbf{return} \texttt{false}\;
$\textup{llNode*} \ node := list$.\texttt{llFind}($key$)\;
\label{alg9:line130}
\If{$node \rightarrow key = key$}
{
    \textbf{return} $list$.\texttt{llInsert}($key$, -1)\;
    \label{alg9:line132}
}
\textbf{else} \textbf{return} \texttt{true}\;
\end{algorithm}


==> algorithm/delete_tree.tex <==
\begin{figure}[H]
% \algrenewcommand\ALG@beginalgorithmic{\footnotesize} % Adjust the font size if needed
\algrenewcommand\alglinenumber[1]{\scriptsize #1:} % Adjust the font size and formatting of the line number

\newcommand{\algrule}[1][.5pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip} 
\begin{multicols}{2}
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
\label{insert}
\algrestore{insert}
\scriptsize
\Statex
\Procedure{\textbf{Delete}}{key}
\State{\texttt{retry}:}
\State{$\textup{Node* } curr := root$}
\If{$curr =$ \textup{\texttt{nullptr}}}
    \State{\textbf{return} \textup{"Key Not Present"}} 
\EndIf
\State{$curr :=$ \textup{\texttt{balanceRoot(curr)}}}
\label{alg:del:balance_root}
\If{{\textup{!}}$\,curr$}{\textup{ \textbf{goto} \texttt{retry}}}
\EndIf
\State{$\textup{Node* } prev, child :=$ \texttt{nullptr}}
\State{int $pidx, cidx$}
\While{\textup{!}$curr \rightarrow isLeaf$}
    \label{alg:del:isleaf}
    \If{$curr \rightarrow helpIdx \neq -1$}
        \label{alg2:line48}
        \label{alg:del:help}
        \State{$\textup{Node*} \, res:=$ \texttt{help}($prev, pidx, curr$)}
        \If{$res$} {$curr := res$}
        \Else { \textup{\textbf{goto} \texttt{retry}}}
        \EndIf
    \EndIf
    % \label{alg:del:}
    \State{{$cidx$ \textup{is set to the index of appropriate child based on} $key$ using Binary Search}}
    \label{alg:del:curridx}
    \State{$child := curr \rightarrow ptr[cidx]$}
    \If{$child\rightarrow isLeaf  \,\&\&\ child\rightarrow frozen$}
        \State{$\,curr \rightarrow$ \texttt{freezeInternal()}}
        % \label{alg1:line20}
        \If{\textup{!}$\,curr \rightarrow$\textup{\texttt{setHelpIdx$(cidx)$}}} 
        \State{\textup{\textbf{goto} \texttt{retry}}}
        
        \EndIf
        \State{$\textup{Node*} newNode:=child\rightarrow$ \texttt{balanceLeaf}($prev, pidx, curr, cidx)$}
        % \label{alg1:line23}
        \If{$newNode$} \State{\textbf{then} $curr := newNode$}
        % \label{alg1:line24}
        \Else{ \textup{\textbf{goto}        \texttt{retry}}}
        % \label{alg1:line25}
        \EndIf
       
    \ElsIf{\textup{!}$\,child \rightarrow isLeaf \&\&\ child \rightarrow count \leq MIN$}
    {
        % \label{alg1:line26}
        \State{$\,curr \rightarrow$ \texttt{freezeInternal()}}
        % \label{alg1:line27}
        \If{\textup{!}$\,curr\rightarrow$\textup{\texttt{setHelpIdx$(cidx)$}}} {
         \State{\textup{\textbf{goto} \texttt{retry}}}
            % \label{alg1:line29}
        }
        \EndIf
        \State{$\textup{Node* } newNode := child \rightarrow$ \texttt{mergeInternal}($prev, pidx, curr, cidx)$}
        % \label{alg1:line30}
        \If{$newNode$} \State{\textbf{then} $curr := newNode$}
        % \label{alg1:line24}
        \Else{ \textup{\textbf{goto}        \texttt{retry}}}
        % \label{alg1:line25}
        \EndIf
    }
    \EndIf
     
    \State{$prev := curr$}
    \State{$curr := child$}
    % \label{alg1:line34}
    \State{$pidx := cidx$}

\EndWhile

\State{$res:=$ $curr \rightarrow$ \textup{\texttt{deleteLeaf}}($key$)}
% \label{alg1:insert_tree}
\If{$res = $ \textup{Failed}}
    \State{\textup{\textbf{goto}        \texttt{retry}}}
\Else{ \textbf{return} \textup{res}}
\EndIf
% \If{$curr \rightarrow$ \textup{\texttt{insertIntoLeaf}}($key, value$)}
% {
    % \label{alg1:line36}
    % \textup{\textbf{return}}\;
% }
% \textbf{else} \textup{\textbf{goto} \texttt{retry}}\;
% \label{alg1:line38}

\EndProcedure
\algstore{delete}
\end{algorithmic}
\end{multicols}
\caption{Pseudocode of \remove operation}
\label{alg:insert}
\end{figure}


==> algorithm/do_helping.tex <==
\begin{algorithm}[H]
\label{dohelping}
\caption{\texttt{help}(prevNode,\ prevIdx,\ currNode)}
$\textup{Node* } currChild := currNode \rightarrow ptr[currNode \rightarrow helpIdx]$\;
\textbf{if} $currChild \rightarrow isLeaf$ \textbf{then} \textbf{return} \texttt{$currChild \rightarrow$ \texttt{balanceLeaf}($prevNode,\ prevIdx,\ currNode,\ currIdx)$}\;
\textbf{else if} $currChild \rightarrow count \geq MAX$ \textbf{then} \textbf{return} \texttt{$currChild \rightarrow$ \texttt{splitInternal}($prevNode,\ prevIdx,\ currNode,\ curr_idx)$}\;
\textbf{else} \textbf{return} \texttt{$currChild \rightarrow$ \texttt{merge}($prevNode,\ prevIdx,\ currNode,\ currIdx)$}\;
\end{algorithm}

==> algorithm/experiment_design.tex <==
\begin{enumerate}
    \item Data structures: Kanva, Finindex, C-IST, AB-Tree (preferably PPoPP 22) 
    \item Index building cost.
    \item Zipf with 0 and 1 factor, threads: 8, 16, 32, 64, 128. (50, 25, 25 and 90, 5, 5) (Standard, Fig 12 ABTree, 2 rows only). In each case output the bash command result in a file that includes cache misses. 
    \item YCSB (Zipf .5, 50\% read, 25\% update, 25\% delete) (Fig 13 ABTree)
    \item Zipf with 0 and 1 factor, thread=64, average after every 5 seconds, (50, 30, 20) 
    \item Other datasets, thread=64, average for 10 seconds, (50, 30, 20) insert and search after insert (Fig 10 FIndex)
    \item Zipf with 1 factor Hotspot 10\%, 25\%, 50\%, 75\% insert and search after insert (Fig 11 Finindex). (10M train samples+ rest test samples).
    \item Experiment with small dataset: $2^10$
    
\end{enumerate}

==> algorithm/insert.tex <==
\begin{algorithm}
\caption{\texttt{\textbf{Insert}} (key, value)}
\label{insert}
\footnotesize

$ix := models \rightarrow find\_idx(key)$\;
\If{keys[ix] = key }
{
    \If{vals[ix] = tombstone}
    {
        update the value of the key\;
        \label{insert:value}
        \texttt{\textbf{return}} true
    }
    \Else{\textbf{return} false}
}
\Else{
    \texttt{retry}:\\
    $current\_level\_bin :=  level\_bin[ix]$\;
    \If{$current\_level\_bin == null$}
    {
    %   $new\_level\_bin := level\_bins[ix]$\;
    %   \If{$new\_level\_bin = null$}{
       $new\_level\_bin$ := new Bin()\;
       \label{newlevelbinstart}
       $new\_level\_bin \rightarrow is\_node := false$\;
       $new\_level\_bin \rightarrow child\_bin :=$ new Child\_Bin()\;
       \label{newlvwlbinend}
       \scriptsize
       $level\_bin[ix].\texttt{\textbf{CAS}}(current\_level\_bin, new\_level\_bin)$\;
       \footnotesize
       \label{levelcas}
       \texttt{\textbf{goto}} retry\;
       \label{insertretry1}
    %   }
    }
    \ElseIf{$current\_level\_bin\rightarrow is\_node$}
    {
        \texttt{\textbf{return}} $current\_level\_bin \rightarrow child\_node \rightarrow insert(key, value)$
    }
    \Else{
        \If{$current\_level\_bin\rightarrow child\_bin \rightarrow size \geq threshold$}{
        $new\_level\_bin := Bin()$\;
        $new\_level\_bin \rightarrow is\_model := true$\;
        $current\_level\_bin\rightarrow bin \rightarrow freeze()$\;
        $bin\_keys, bin\_vals := current\_level\_bin\rightarrow bin \rightarrow collect()$\;
       $new\_level\_bin \rightarrow child\_node :=$ new Node(keys,vals)\;
       \tiny
       $level\_bin[ix].\texttt{\textbf{CAS}}(current\_level\_bin, new\_level\_bin)$\;
       \footnotesize
       \texttt{\textbf{goto}} retry\;
        }
        % \tiny
        \Else
        {   
            res := $current\_level\_bin\rightarrow bin \rightarrow insert(key,value)$ \;
            \footnotesize
            \If{res = frozen}
            {
                \textbf{goto} retry\;
            }
            \Else{
            \texttt{\textbf{return} res}
            }
            % \texttt{\textbf{return} res} 
        }
    }
}
\end{algorithm}

==> algorithm/insert_leaf.tex <==
\begin{figure}[H]
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\begin{multicols}{2}
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}\scriptsize
\algrestore{rangequery}
\Procedure{\textbf{insertLeaf}}{key,value}

% \begin{algorithm}[H]
% \label{insertintoleaf}
% \caption{\texttt{insertIntoLeaf}(key,\ value)}
\If{$frozen$}{ \textbf{return} \texttt{"Failed"}}
\EndIf
\label{alg5:line97}
\If{$count \geq MAX$}
% {
    \State{\texttt{freezeLeaf()}}
    \label{alg5:line99}
    \State{\textbf{return}
    \texttt{"Failed"}}
    \label{alg5:line100}
% }
\Else
    \State{res := \texttt{\textup{llInsert}}($key,\ value$)}
    \If{res = "New Key Inserted"}
% {
    \label{alg5:line101}
    \State{$count$++}
    \EndIf
    % \State{\textbf{return} res 
    \State{\textbf{return} res}
    
\EndIf
% }
% \State{\textbf{return} \texttt{false}}
\EndProcedure
\algstore{insertleaf}
% \end{algorithm}
\end{algorithmic}
\hrule
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}\scriptsize
\algrestore{insertleaf}
% \State{\hrulefill}
\Procedure{\textbf{deleteLeaf}}{key}
% \caption{\texttt{deleteFromLeaf}(key)}
\State{$\textup{llNode*} node :=$ \texttt{find}($key$)}
\label{alg9:line130}
\If{$node \rightarrow key = key$}
% {
    \State{res := \texttt{insert}($key$, tombstone)}
    \label{alg9:line132}
    \State{\textbf{return} \texttt{res}}
\EndIf
% }
\State{\textbf{return} \texttt{"Key Not Present"}}
\EndProcedure
\algstore{deleteleaf}
\end{algorithmic}
\hrule
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}\scriptsize
\algrestore{deleteleaf}
% \State{\hrulefill}
\Procedure{\textbf{balanceRoot}}{currRoot}
% \caption{\texttt{balanceRoot}()}
\State{$\textup{Node* } newNode$}
\If{$currRoot \rightarrow isLeaf\ \&\&\ currRoot \rightarrow frozen$}
% {
     \If{$currRoot \rightarrow count \geq MAX$} {$newNode :=$ \texttt{splitRootLeaf}()}
    \Else { $newNode :=$ \texttt{createNewLeaf}()}
    \EndIf
\ElsIf {\textup{!}$currRoot \rightarrow isLeaf\ \&\&\ currRoot \rightarrow count \geq MAX$}{ $newNode :=$ \texttt{splitRootInternal}()}
\EndIf
\If{\textup{!}$\,root$.\texttt{CAS}($\textit{\textit{\textbf{this}}},\  newNode$)} {\textup{\textbf{return}} \texttt{nullptr}}
\Else{ \textbf{\textup{return}} $newNode$}
\EndIf
\EndProcedure
\algstore{balanceroot}
\end{algorithmic}
\hrule

\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}\scriptsize
\algrestore{balanceroot}
% \State{\hrulefill}
\Procedure{\textbf{balanceLeaf}}{prevNode,\ prevIdx,\ currNode,\ currIdx}

% \caption{\texttt{balanceLeaf}(prevNode,\ prevIdx,\ currNode,\ currIdx)}
\If{ $currNode \rightarrow helpIdx \neq$ -1} 
\State{\textbf{return} \texttt{nullptr}}
\ElsIf{\textup{!}$\,currNode \rightarrow helpIdx$.\texttt{CAS}(-1, $currIdx$)}
\State{\textbf{return} \texttt{nullptr}}
\EndIf
\State{$\textup{Node* } newNode$}
\If{$count \geq MAX$} 
% {
    \State{$newNode :=$ \texttt{splitLeaf}($prevNode,$ $\ prevIdx,$ $\ currNode,\ currIdx$)}
    \label{alg8:line122}
% }
\ElsIf{$count < MIN$}
% {
    \State{$newNode :=$ \texttt{merge}($prevNode,$ $\ prevIdx,\ currNode,\ currIdx$)}
    \label{alg8:line124}
% }
\Else
% {
    \State{$newNode :=$ \texttt{createNewLeaf}($prevNode,$ $\ prevIdx,$ $\ currNode,\ currIdx$)}
    \label{alg8:line126}
% }
\EndIf
\State{\textbf{return} $newNode$}

\EndProcedure
\algstore{balanceleaf}
\end{algorithmic}


\hrule
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}\scriptsize
\algrestore{balanceleaf}
% \State{\hrulefill}
\Procedure{\textbf{help}}{prevNode,\ prevIdx,\ currNode}
% \caption{\texttt{help}(prevNode,\ prevIdx,\ currNode)}
\State{$\textup{Node* } currChild := currNode \rightarrow ptr[currNode \rightarrow helpIdx]$}
\If{$currChild \rightarrow isLeaf$} \State{\textbf{return} \texttt{$currChild \rightarrow$ \texttt{balanceLeaf}($prevNode,\ prevIdx,\ currNode,\ currIdx)$}}
\ElsIf{$currChild \rightarrow count \geq MAX$} 
\State{\textbf{return} \texttt{$currChild \rightarrow$ \texttt{splitInternal}($prevNode,\ prevIdx,\ currNode,\ curr_idx)$}}
\Else 
\State{textbf{return} \texttt{$currChild \rightarrow$ \texttt{merge}($prevNode,\ prevIdx,\ currNode,\ currIdx)$}}
\EndIf
\EndProcedure
\algstore{help}
\end{algorithmic}

\hrule
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}\scriptsize
\algrestore{help}
% \State{\hrulefill}
\Procedure{\textbf{freezeInternal()}}{}
% \caption{\texttt{markInternal()}}
\For{$i := 0$ \textbf{to} $MAX$}
% {
    \State{$ptr[i]$.\texttt{CAS}($ptr[i],\  $ \texttt{markedRef}($ptr[i]))$}
    \label{alg12:line160}
\EndFor
\State{\textit{frozen} := \texttt{True}}
% }
\EndProcedure
\algstore{freezeInternal}

\end{algorithmic}
\hrule
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}\scriptsize
\algrestore{freezeInternal}
% \State{\hrulefill}
\Procedure{\textbf{freezeLeaf()}}{}
\State{llNode* $currNode := ver\_head$}
\While{$currNode \rightarrow next \neq$ \textup{\texttt{nullptr}}}
    \State{$currNode \rightarrow next$.\texttt{CAS}($currNode \rightarrow next,\ $ \texttt{markedRef}($currNode \rightarrow next$))}
    \label{alg13:line163}
    \State{$currNode \rightarrow vhead$.\texttt{CAS}($currNode \rightarrow vhead,\ $ \texttt{markedRef}($currNode \rightarrow vhead$))}
    \label{alg13:line164}
    \State{$currNode := currNode \rightarrow next$}
\EndWhile
\State{$\textit{\textbf{this}} \rightarrow count := list$.\texttt{size()}}
\State{\textit{frozen} := \texttt{True}}
\EndProcedure
\algstore{freezeleaf}
\end{algorithmic}
\end{multicols}
\caption{Pseudocode of insertLeaf, deleteLeaf, balanceRoot, balanceLeaf, help, freezeInternal and freezeLeaf}
\label{fig:freeze}
\end{figure}

==> algorithm/insert_tree.tex <==
\begin{figure}[H]

% \renewcommand{\figurename}{Algorithm}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\begin{multicols}{2}
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
\label{Read}
\scriptsize
\Procedure{\textbf{Insert}}{key, value}
\State{\texttt{retry}:}
\State{$\textup{Node* } curr := root$}
\If{$curr =$ \textup{\texttt{nullptr}}}
    \State{$\textup{Node* }\ nLeaf\rightarrow$\texttt{insLeaf}($key$, $value$)}
    \If{\textup{!}$\,root$.\textup{\texttt{CAS}}($curr, nLeaf$)}
        \label{alg1:line5}
        \State{\textup{\textbf{goto} \texttt{retry}}}
        \label{alg1:line6}
    \Else { \textup{\textbf{return}}}
    \EndIf
\EndIf
\State{$curr :=$ \textup{\texttt{balanceRoot(curr)}}}
\label{alg1:line8}
\If{{\textup{!}}$\,curr$}{\textup{ \textbf{goto} \texttt{retry}}}
\EndIf
\State{$\textup{Node* } prev, child :=$ \texttt{nullptr}}
\State{int $pidx, cidx$}
\While{\textup{!}$curr \rightarrow isLeaf$}
    \label{alg1:line12}
    \If{$curr \rightarrow helpIdx \neq -1$}
        \label{alg1:line13}
        \State{$\textup{Node*} \, res:=$ \texttt{help}($prev, pidx, curr$)}
        \If{$res$} {$curr := res$}
        \Else { \textup{\textbf{goto} \texttt{retry}}}
        \EndIf
    \EndIf
    \label{alg1:line16}
    \State{{$cidx$ \textup{is set to the index of appropriate child based on} $key$ using Binary Search}}
    \label{alg1:line17}
    \State{$child := curr \rightarrow ptr[cidx]$}
    \If{$child\rightarrow isLeaf  \,\&\&\ child\rightarrow frozen$}
        \State{$\,curr \rightarrow$ \texttt{freezeInternal()}}
        \label{alg1:line20}
        \If{\textup{!}$\,curr \rightarrow$\textup{\texttt{setHelpIdx$(cidx)$}}} 
        \State{\textup{\textbf{goto} \texttt{retry}}}
        
        \EndIf
        \State{$\textup{Node*} newNode:=child\rightarrow$ \texttt{balanceLeaf}($prev, pidx, curr, cidx)$}
        \label{alg1:line23}
        \If{$newNode$} \State{\textbf{then} $curr := newNode$}
        \label{alg1:line24}
        \Else{ \textup{\textbf{goto}        \texttt{retry}}}
        \label{alg1:line25}
        \EndIf
       
    \ElsIf{\textup{!}$\,child \rightarrow isLeaf \&\&\ child \rightarrow count \geq MAX$}
    {
        \label{alg1:line26}
        \State{$\,curr \rightarrow$ \texttt{freezeInternal()}}
        \label{alg1:line27}
        \If{\textup{!}$\,curr\rightarrow$\textup{\texttt{setHelpIdx$(cidx)$}}} {
         \State{\textup{\textbf{goto} \texttt{retry}}}
            \label{alg1:line29}
        }
        \EndIf
        \State{$\textup{Node* } newNode := child \rightarrow$ \texttt{splitInternal}($prev, pidx, curr, cidx)$}
        \label{alg1:line30}
        \If{$newNode$} \State{\textbf{then} $curr := newNode$}
        \label{alg1:line24}
        \Else{ \textup{\textbf{goto}        \texttt{retry}}}
        \label{alg1:line25}
        \EndIf
    }
    \EndIf
     
    \State{$prev := curr$}
    \State{$curr := child$}
    \label{alg1:line34}
    \State{$pidx := cidx$}

\EndWhile

\State{$res:=$ $curr \rightarrow$ \textup{\texttt{insertLeaf}}($key, value$)}
\label{alg1:insert_tree}
\If{$res = $ \textup{Failed}}
    \State{\textup{\textbf{goto}        \texttt{retry}}}
\Else{ \textbf{return} \textup{res}}
\EndIf
% \If{$curr \rightarrow$ \textup{\texttt{insertIntoLeaf}}($key, value$)}
% {
    % \label{alg1:line36}
    % \textup{\textbf{return}}\;
% }
% \textbf{else} \textup{\textbf{goto} \texttt{retry}}\;
% \label{alg1:line38}
% 
\EndProcedure
\algstore{insert}
\end{algorithmic}
\end{multicols}
\caption{Pseudocode of \insertADT operation}
\label{alg:insert}
% \label{alg:insert}
\end{figure}


==> algorithm/linked_list/WFinsert_ll.tex <==
\begin{algorithm}[H]
\label{WFllinsert}
\caption{\texttt{wfLLInsert}(key, value, tid, phase)}
\While{\textup{\texttt{true}}}
{
    llNode* $prevNode :=$ \texttt{nullptr}\;
    llNode* $nextNode :=$ \texttt{llFind}($key,\  \&prevNode$)\;
    \If{$nextNode ==$ \textup{\texttt{nullptr}}}
    {
        \textbf{return} \texttt{false}\;
    }
    \ElseIf{$nextNode \rightarrow key == key$}
    {
        \While{\textup{\texttt{true}}}
        {
            $currState := stateArray[tid]$\;
            \label{alg25:line294}
            \textbf{if} $currState \rightarrow finished$ || $currState \rightarrow phase \neq phase$  \textbf{then return} \texttt{true} \;\label{alg25:line295}
            $newVnode := currState \rightarrow vNode$\;
            \label{alg25:line296}
            $nextVnode := newVnode \rightarrow nextv$\;
            \label{alg25:line297}
            $currVhead := nextNode \rightarrow vhead$\;
            \label{alg25:line298}
             \texttt{initTs}($currVhead)$\;
             \label{alg25:init}
             $currValue := currVhead \rightarrow value$\;
            \label{alg25:line303}
            
            \If{$currState \rightarrow vnode \rightarrow ts \neq$ -1}
            {
                \label{alg25:line300}
                $currState \rightarrow finished =$ \texttt{true}\;
                \textbf{return} \texttt{true}\;
                \label{alg25:line302}
            }
            \textbf{if} \texttt{isMarked}($currVhead$) \textbf{then} \textbf{return} \texttt{false} \;
            \If{\textup{\texttt{wfVCAS}}($nextNode,\ currValue,\ value,\ newVnode,\ \newline
            nextVnode,\ currVhead  $)}{
            \label{alg25:line304}
            $currState \rightarrow finished := true$\;
            \textbf{return} \texttt{true}
            }
        }
    }
    \Else
    {
        $currState := stateArray[tid]$\;
        \textbf{if} $currState \rightarrow finished$ \textbf{then return} \texttt{true} \;\label{alg25:line308}
        \If{$phase \neq currState \rightarrow phase\  \&\& \ currState \rightarrow vnode \rightarrow ts \neq$ -1}
            {
                \label{alg25:line309}
                $currState \rightarrow finished =$ \texttt{true}\;
                \textbf{return} \texttt{true}\;
            }
        llNode* $newNode :=$ \texttt{new llNode}($key,\ value,\ currState \rightarrow vnode$)\;
        $newNode \rightarrow next := nextNode$\;
        \If{$prevNode \rightarrow next$.\textup{\texttt{CAS}}($nextNode,\ newNode$)}{
        \label{alg25:line314}
            \texttt{initTs}$(newNode \rightarrow vhead)$\;
            \label{alg25:line312}
            $currState \rightarrow finished := true$
            \textbf{return} \texttt{true}\;
        }
        \textbf{else if} \texttt{isMarked}($prevNode \rightarrow next$) \textbf{then return} \texttt{false}\;
    }
}
\end{algorithm}

==> algorithm/linked_list/find_ll.tex <==
\begin{figure}
\begin{multicols}{2}
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{}
\scriptsize
\algrestore{wfdeleteleaf}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\Procedure{\textbf{llFind}}{key, prevNode}
% \label{llfind}
% \caption{\texttt{llFind}(key, prevNode)}
\State{$prevNode := head$}
\While{\textup{\texttt{true}}}
% {
    \State{llNode* $rightNode := prevNode \rightarrow next$}
    \label{alg20:line243}
    \If{\textup{\texttt{isMarked}}$(rightNode)$}
    % {
        \State{ \textbf{return}\texttt{nullptr}}
    % }
    \ElsIf{$rightNode \rightarrow key \geq key$}
    % {
        \State{\textbf{return} $rightNode$}
    % }
    \Else
    % {
        \State{$prevNode := rightNode$}
    % }
    \EndIf
% }
\EndWhile
\EndProcedure
\algstore{llfind}
\end{algorithmic}
\hrule

  \begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{}
\scriptsize
\algrestore{llfind}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\Procedure{\textbf{initTs}}{Vnode}
% \caption{\texttt{initTs}(Vnode)}
\If{$Vnode \rightarrow ts =$ -1}
% {
    % \State{$currTs :=$ \texttt{getCurrTs()}}
    \State{$Vnode \rightarrow ts$.\texttt{CAS}(-1, $currTs)$}
    \label{alg22:line270}
    \EndIf
% }
\EndProcedure
\algstore{inits}
\end{algorithmic}



\hrule

  \begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{}
\scriptsize
\algrestore{inits}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\Procedure{\textbf{read}}{llNode}
% \caption{\texttt{initTs}(Vnode)}
% \caption{\texttt{read}(llNode)}
\State{$currVhead := llNode \rightarrow vhead$}
\State{\texttt{initTs}$(currVhead)$}
\label{alg23:line272}
\State{\textbf{return} $currVhead \rightarrow value$}
\EndProcedure
\algstore{read}
\end{algorithmic}
\hrule
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{}
\scriptsize
\algrestore{read}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\Procedure{\textbf{vCAS}}{currNode, oldValue, value}
% \caption{\texttt{initTs}(Vnode)}
% \caption{\texttt{read}(llNode)}
\State{$currVhead :=$ \texttt{unmarkedRef}$(currNode \rightarrow vhead)$}
\State{\texttt{initTs}$(currVhead)$} 
\label{alg24:line275}
\If{$currVhead \rightarrow value \neq oldValue$}
\State{\textbf{return} \texttt{false}}
\EndIf
\If{$currVhead \rightarrow value = newValue$}
\State{\textbf{return} \texttt{true}}
\EndIf
\State{Vnode* $newVnode :=$ \texttt{new Vnode}$(value)$}
\State{$newVnode \rightarrow nextv := currVhead$}
\If{$currNode \rightarrow vhead$.\texttt{CAS}$(currVhead,$ $\ newVnode)$}
% {
    \label{alg24:line280}
    \State{\texttt{initTs}$(newVnode)$} \label{alg24:line281}
    \State{\textbf{return} \texttt{true}}
    
% }
\Else 
\State{\texttt{initTs}$(currNode \rightarrow vhead)$}
\State{\textbf{return} \texttt{false}}
\EndIf
\EndProcedure
\algstore{vcas}
\end{algorithmic}

\hrule
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{}
\scriptsize
\algrestore{vcas}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\Procedure{\textbf{wfVCAS}}{currNode, oldValue, value, newVnode, nextVnode, currVhead}
\If{$currVhead \rightarrow value \neq oldValue$}
\State{\textbf{return} \texttt{false}}
\EndIf
\If{ $currVhead \rightarrow value = newValue$}
\State{\textbf{return} \texttt{true}}
\EndIf
\If{$\, !\, (newVnode \rightarrow nextv.$\texttt{CAS}$(nextVnode,$ $ currVhead))$}
\State{\textbf{return} \texttt{false}}
\label{alg26:line320}
\EndIf
\If{$currNode \rightarrow vhead$.\textup{\texttt{CAS}}$(currVhead,$ $\ newVnode)$}
% {
    \label{alg26:line321}
    \State{\texttt{initTs}$(newVnode)$}
     \label{alg26:line319}
    \State{\textbf{return} \texttt{true}}
% }
\Else
\State{\texttt{initTs}$(currNode \rightarrow vhead)$}
\State{\textbf{return} \texttt{false}}
\EndIf
\EndProcedure
\algstore{wfvcas}
\end{algorithmic}



\end{multicols}
\caption{Pseudocode of llFind, initTs, read, vCAS and wfVCAS}
\label{llfind}
\end{figure}











\begin{figure}
    \begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{}
\scriptsize
\algrestore{wfvcas}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\Procedure{\textbf{llInsert}}{key, value}
% \caption{\texttt{llInsert}(key, value)}
\While{\textup{\texttt{true}}}
% {
    \State{llNode* $prevNode :=$ \texttt{nullptr}}
    \State{llNode* $nextNode :=$ \texttt{find}($key,$ $\&prevNode$)}
    \label{alg21:line252}
    \If{$nextNode =$ \textup{\texttt{nullptr}}}
    % {
        \State{\textbf{return} \texttt{"Failed"}}
    % }
    \ElsIf{$nextNode \rightarrow key = key$}
    % {
        \While{\textup{\texttt{true}}}
        % {
            \State{$currVhead := nextNode \rightarrow vhead$}
            \If{\texttt{isMarked}($currVhead$)} 
            \State{\textbf{return} \texttt{"Failed"}}
            \EndIf
            \State{$currValue :=$ \texttt{read}($currVhead)$}
            \If{\texttt{vCAS}($nextNode,\ currValue,$ $\ value,\ currVhead $) }
            \State{\textbf{return} \texttt{"Key Updated"}}
            \label{alg21:line260}
            \EndIf
        % }
        \EndWhile
    % }
    \Else
    % {
        \State{llNode* $newNode :=$ \texttt{new llNode}($key,\ value$)}
        \State{$newNode \rightarrow next := nextNode$}
        \If{$prevNode \rightarrow next$.\textup{\texttt{CAS}}($nextNode,\ newNode$)}
        % {
            \label{alg21:line264}
            \State{\texttt{initTs}$(newNode \rightarrow vhead)$}
            \label{alg21:line265}
            \State{\textbf{return} \texttt{"New Key Inserted"}}
        % }
        \ElsIf{\texttt{isMarked($prevNode \rightarrow next$)}} \State{\textbf{return} \texttt{"Failed"}}
        \EndIf
    % }
    \EndIf
% }
\EndWhile
\EndProcedure
\algstore{llinsert}
\caption{Pseudocode of Linked-List Insert}

\label{llinsert}
% \EndWhile
\end{algorithmic}
\end{figure}


\begin{figure}
    \begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{}
\scriptsize
\algrestore{llinsert}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\Procedure{\textbf{wfLLInsert}}{key, value, tid, phase}
% \caption{\texttt{llInsert}(key, value)}
\While{\textup{\texttt{true}}}
% {
    \State{llNode* $prevNode :=$ \texttt{nullptr}}
    \State{llNode* $nextNode :=$ \texttt{find}($key,\  \&prevNode$)}
    \If{$nextNode ==$ \textup{\texttt{nullptr}}}
    % {
        \State{\textbf{return} \texttt{"Failed"}}
    % }
    \ElsIf{$nextNode \rightarrow key = key$}
    % {
        \While{\textup{\texttt{true}}}
        % {
            \State{$currState := stateArray[tid]$}
            \label{alg25:line294}
            \If{$currState \rightarrow finished$}
            \State{\textbf{return} \texttt{"Operation Finished"}} \label{alg25:line295}
            \EndIf
            \State{$newVnode := currState \rightarrow vNode$}
            \label{alg25:line296}
            \State{$nextVnode := newVnode \rightarrow nextv$}
            \label{alg25:line297}
            \State{$currVhead := nextNode \rightarrow vhead$}
            \label{alg25:line298}
             \State{\texttt{initTs}($currVhead)$}
             \label{alg25:init}
             \State{$currValue := currVhead \rightarrow value$}
            \label{alg25:line303}
            
            \If{$phase \neq currState \rightarrow phase\  \&\& \ currState \rightarrow vnode \rightarrow ts \neq$ -1}
            % {
                \label{alg25:line300}
                \State{$currState \rightarrow finished =$ \texttt{true}}
                \State{\textbf{return} \texttt{"Operation Finished"}}
                \label{alg25:line302}
            % }
            \EndIf
            \If{\texttt{isMarked}($currVhead$)}
            \State{\textbf{return} \texttt{"Failed"}}
            \EndIf
            \If{\textup{\texttt{wfVCAS}}($nextNode,\ currValue,\ value,\ newVnode,\
            nextVnode,\ currVhead  $)}
            
            \label{alg25:line304}
            \State{\textbf{return} \texttt{"Key Updated"}}
            % }
            \EndIf
        % }
        \EndWhile
    \Else
    % {
        \State{$currState := stateArray[tid]$}
        \If{$currState \rightarrow finished$}
        \State{\textbf{return} \texttt{"Operation Finished"}} \label{alg25:line308}
        \EndIf
        \If{$phase \neq currState \rightarrow phase\  \&\& \ currState \rightarrow vnode \rightarrow ts \neq$ -1}
            % {
                \label{alg25:line309}
                \State{$currState \rightarrow finished =$ \texttt{true}}
                \State{\textbf{return} \texttt{"Operation Finished"}}
            % }
        \EndIf    
        \State{llNode* $newNode :=$ \texttt{new llNode}($key,\ value,\ currState \rightarrow vnode$)}
        \State{$newNode \rightarrow next := nextNode$}
        \If{$prevNode \rightarrow next$.\textup{\texttt{CAS}}($nextNode,\ newNode$)}
        % {
        \label{alg25:line314}
            \State{\texttt{initTs}$(newNode \rightarrow vhead)$}
            \label{alg25:line312}
            \State{$currState \rightarrow finished := true$}
            \State{\textbf{return} \texttt{"New Key Inserted"}}
        
        \ElsIf{\texttt{isMarked}($prevNode \rightarrow next$)}
        \State{\textbf{return} \texttt{"Failed"}}
        \EndIf
    % }
    \EndIf
% }
\EndWhile
\EndProcedure
\algstore{wfllinsert}

% \EndWhile
\end{algorithmic}
\caption{Pseudocode of wait-free Linked-List Insert}
\label{wfllinsert}
\end{figure}

==> algorithm/linked_list/init_ts.tex <==
\begin{algorithm}[H]
\label{llinit_ts}
\caption{\texttt{initTs}(Vnode)}
\If{$Vnode \rightarrow ts =$ -1}
{
    $currTs :=$ \texttt{getCurrTs()}\;
    $Vnode \rightarrow ts$.\texttt{CAS}(-1, $currTs)$\;
    \label{alg22:line270}
}
\end{algorithm}

==> algorithm/linked_list/insert_ll.tex <==
\begin{algorithm}[H]
\label{llinsert}
\caption{\texttt{llInsert}(key, value)}
\While{\textup{\texttt{true}}}
{
    llNode* $prevNode :=$ \texttt{nullptr}\;
    llNode* $nextNode :=$ \texttt{llFind}($key,\  \&prevNode$)\;
    \label{alg21:line252}
    \If{$nextNode =$ \textup{\texttt{nullptr}}}
    {
        \textbf{return} \texttt{false}\;
    }
    \ElseIf{$nextNode \rightarrow key = key$}
    {
        \While{\textup{\texttt{true}}}
        {
            $currVhead := nextNode \rightarrow vhead$\;
            \textbf{if} \texttt{isMarked}($currVhead$) \textbf{then} \textbf{return} \texttt{false} \;
            $currValue :=$ \texttt{read}($currVhead)$\;
            \textbf{if}\texttt{vCAS}($nextNode,\ currValue,\ value,\ currVhead $) \textbf{then} \textbf{return} \texttt{true}\;
            \label{alg21:line260}
        }
    }
    \Else
    {
        llNode* $newNode :=$ \texttt{new llNode}($key,\ value$)\;
        $newNode \rightarrow next := nextNode$\;
        \If{$prevNode \rightarrow next$.\textup{\texttt{CAS}}($nextNode,\ newNode$)}{
            \label{alg21:line264}
            \texttt{initTs}$(newNode \rightarrow vhead)$\;
            \label{alg21:line265}
            \textbf{return} \texttt{true}\;
        }
        \textbf{else if} \texttt{isMarked}($prevNode \rightarrow next$) \textbf{then return} \texttt{false}\;
    }
}
\end{algorithm}

==> algorithm/linked_list/read.tex <==
\begin{algorithm}[H]
\label{llread}
\caption{\texttt{read}(llNode)}
$currVhead := llNode \rightarrow vhead$\;
\texttt{initTs}$(currVhead)$\;
\label{alg23:line272}
\textbf{return} $currVhead \rightarrow value$\;
\end{algorithm}


==> algorithm/linked_list/vCAS.tex <==
\begin{algorithm}[H]
\label{llvcas}
\caption{\texttt{vCAS}(currNode, oldValue, value)}
$currVhead :=$ \texttt{unmarkedRef}$(currNode \rightarrow vhead)$\;
\texttt{initTs}$(currVhead)$\; 
\label{alg24:line275}
\textbf{if} $currVhead \rightarrow value \neq oldValue$ \textbf{then return} \texttt{false}\;
\textbf{if} $currVhead \rightarrow value = newValue$ \textbf{then return} \texttt{true}\;
Vnode* $newVnode :=$ \texttt{new Vnode}$(value)$\;
$newVnode \rightarrow nextv := currVhead$\;
\If{$currNode \rightarrow vhead$.\texttt{CAS}$(currVhead,\ newVnode)$}
{
    \label{alg24:line280}
    \texttt{initTs}$(newVnode)$\; \label{alg24:line281}
    \textbf{return} \texttt{true}\;
}
\textbf{else return} \texttt{false}\;
\end{algorithm}

==> algorithm/linked_list/wfVCAS.tex <==
\begin{algorithm}[H]
\label{wfllvcas}
\caption{\texttt{wfVCAS}(currNode, oldValue, value, newVnode, nextVnode, currVhead )}
\textbf{if} $currVhead \rightarrow value \neq oldValue$ \textbf{then return} \texttt{false}\;
\textbf{if} $currVhead \rightarrow value = newValue$ \textbf{then return} \texttt{true}\;
\textbf{if}$\, !\, (newVnode \rightarrow nextv.$\texttt{CAS}$(nextVnode, currVhead))$ \textbf{then return} \texttt{false}\;
\label{alg26:line320}
\If{$currNode \rightarrow vhead$.\textup{\texttt{CAS}}$(currVhead,\ newVnode)$}
{
    \label{alg26:line321}
    \texttt{initTs}$(newVnode)$\;
     \label{alg26:line319}
    \textbf{return} \texttt{true}\;
}
\textbf{else return} \texttt{false}\;
\end{algorithm}

==> algorithm/mark_internal.tex <==
\begin{algorithm}[H]
\label{markinternal}
\caption{\texttt{freezeInternal()}}
\For{$i := 0$ \textbf{to} $MAX$}
{
    
    $ptr[i]$.\texttt{CAS}($ptr[i],\  $ \texttt{markedRef}($ptr[i]))$\;
    \label{alg12:line160}
}
$frozen := true$\;
\end{algorithm}

==> algorithm/mark_leaf.tex <==
\begin{algorithm}[H]
\label{markleaf}
\caption{\texttt{freezeLeaf()}}
llNode* $currNode := list.head$\;
\While{$currNode \rightarrow next \neq$ \textup{\texttt{nullptr}}}
{
    $currNode \rightarrow next$.\texttt{CAS}($currNode \rightarrow next,\ $ \texttt{markedRef}($currNode \rightarrow next$))\;
    \label{alg13:line163}
    $currNode \rightarrow vhead$.\texttt{CAS}($currNode \rightarrow vhead,\ $ \texttt{markedRef}($currNode \rightarrow vhead$))\;
    \label{alg13:line164}
    $currNode := currNode \rightarrow next$\;
}
$frozen := true$\;
$count := list$.\texttt{size()}\;
\end{algorithm}

==> algorithm/merge.tex <==
\begin{figure}[H]

% \renewcommand{\figurename}{Algorithm}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\begin{multicols}{2}
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
\label{merge}
\scriptsize
\algrestore{freezeleaf}
\Procedure{\textbf{merge}}{prev,\ pidx,\ curr,\ cidx}
% \label{merge}
% \caption{\texttt{merge}(prev,\ pidx,\ curr,\ cidx)}
\State{int $lsIdx := cidx$ - 1}
\State{int $rsIdx := cidx$ + 1}
\If{$lsIdx \geq 0$}
    \State{$\textup{Node* } lChild := curr \rightarrow ptr[lsIdx]$}
    \If{$lChild \rightarrow$ isLeaf }
    \State{$lChild \rightarrow$ freezeLeaf}
    \label{alg14:line171}
    \Else
    \State{$lChild \rightarrow$ freezeInternal}
    \EndIf
    
    \State{\textbf{return} \texttt{mergeHelper}($\textit{\textbf{this}},$ $\ cidx,\ leftChild,$ $ lsIdx,\ $ $ prev,\ pidx,\ curr)$}
\ElsIf{$rsIdx \leq curr \rightarrow count$}
    \State{$\textup{Node* } rChild := curr \rightarrow ptr[rsIdx]$}
    \If{$lChild \rightarrow$ isLeaf}
    \State{$rChild \rightarrow$ freezeLeaf}
    \label{alg14:line175}
    \Else
    \State{$rChild \rightarrow$ freezeInternal}
    \EndIf
    \State{\textbf{return} \texttt{mergeHelper}($rChild, $ $\ rsIdx,\ \textit{\textbf{this}}, $ $\ cidx,\ prev,$ $ \ pidx,\ curr)$}

\EndIf
\EndProcedure
\algstore{merge}
\end{algorithmic}
\hrule 
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{splitInternal}
\scriptsize
\algrestore{merge}
\Procedure{\textbf{splitInternal}}{prevNode,\ prevIdx,\ currNode,\ currIdx}
% \label{splitinternal}
% \caption{\texttt{splitInternal}(prevNode,\ prevIdx,\ currNode,\ currIdx)}
\State{\texttt{markInternal()}}
\State{$\textup{Node* } lChild :=$ \texttt{new internalNode()}}
\State{\textup{Node* } rChild := \texttt{new internalNode()}}
\State{Split \textbf{\textit{this}} node into a pair of nodes pointed to by $lChild$ and $rChild$}
\State{$\textup{Node* } newNode :=$ \texttt{new internalNode()}}
\State{Copy elements from $currNode$ to $newNode$ replacing $currChild$ with the two pointers $lChild$ and $rChild$}
\If{$prevNode =$ \textup{\texttt{nullptr}}}
% {
    \If{\textup{!}$\,root$.\texttt{CAS}($currNode,\ newNode$)} \State{\textbf{return} \texttt{nullptr}}
    \EndIf 
% }
\ElsIf {!$\,prevNode \rightarrow ptr[prevIdx]$.\texttt{CAS} ($currNode, newNode$)} 
\State{\textbf{return} \texttt{nullptr}}
\EndIf
\State{\textbf{return} $newNode$}
\EndProcedure
\algstore{splitinternal}
\end{algorithmic}

\hrule
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{splitInternal}
\scriptsize
\algrestore{splitinternal}
\Procedure{\textbf{splitLeaf}}{prevNode,\ prevIdx,\ currNode,\ currIdx}

% \caption{\texttt{splitLeaf}(prevNode,\ prevIdx,\ currNode,\ currIdx)}
\State{$\textup{Node* } lChild :=$ \texttt{new leafNode()}}
\State{$\textup{Node* } rChild :=$ \texttt{new leafNode()}}
\State{Split \textit{\textbf{this}} node into a pair of nodes pointed to by $lChild$ and $rChild$}
\label{alg19:line233}
\If{\textup{!}$newNext$.\texttt{\textup{CAS}}($nullptr,lChild$)}
% {
    \label{alg19:line234}
    \State{$lChild := newNext$}
    \State{$rChild := leftChild \rightarrow next$}
% }
\EndIf
\State{$lChild \rightarrow next := rChild$}
\label{alg19:line237}
\State{$\textup{Node* } newNode :=$ \texttt{new internalNode()}}
\State{Copy elements from $currNode$ to $newNode$ replacing $currChild$ with the two pointers $lChild$ and $rChild$}
\label{alg19:line239}
\If{$prevNode =$ \textup{\texttt{nullptr}}}
% {
    \If{\textup{!}$\,root$.\texttt{CAS}($currNode,\ newNode$)}
    \State{\textbf{return} \texttt{nullptr}} \label{alg19:line241}
    \EndIf
% }
\ElsIf{!$\,prevNode \rightarrow ptr[prevIdx]$.\texttt{CAS} ($currNode,\ newNode$)}
\State{\textbf{return} \texttt{nullptr}} 
\label{alg19:line242}
\EndIf
\State{\textbf{return} $newNode$}

\EndProcedure
\algstore{splitLeaf}
\end{algorithmic}




\end{multicols}
\caption{Pseudocode of merge, splitInternal and splitLeaf \op}
\label{merge}
\end{figure}
% \hrule
% \begin{figure}



==> algorithm/merge_helper.tex <==
\begin{algorithm}[H]
\label{mergehelper}
\caption{\texttt{mergeHelper}(rightChild,\ rightIdx,\ leftChild,\ leftIdx,\ prev,\ pidx,\ curr)}
\textup{Node*} $newNode$\;
\If{$rightChild \rightarrow count + leftChild \rightarrow count < MAX$}
{
    \textup{Node*} $newChild$\;
    \If{$leftChild \rightarrow isLeaf$}
    {
        $newChild :=$ \texttt{new LeafNode()}\;
        $newChild \rightarrow next := rightChild \rightarrow next$\;
    }
    \Else
    {
        $newChild :=$ \texttt{new InternalNode()}\;
    }
    Merge $rightChild$ and $leftChild$ into $newChild$\;
    \label{alg15:line185}
    \If{\textup{!}$\,leftChild \rightarrow newNext$.\texttt{\textup{CAS}}(\texttt{\textup{nullptr}}, $newChild$)}
    {
        \label{alg15:line186}
        $newChild := leftChild \rightarrow newNext$\;
    }
    $newNode :=$ \texttt{new InternalNode()}\;
    Copy every element in $curr$ into $newNode$ replacing pointers $leftChild$ and $rightChild$ with $newChild$\;
    \label{alg15:line189}
}
\textbf{else} $newNode :=$ \texttt{borrowHelper}($rightChild,\ rightIdx,\ leftChild,\ leftIdx,\ curr$)\;
\If{$prev =$ \texttt{\textup{nullptr}}}
{
    \If{$newNode \rightarrow count = 0$} 
    {
        $newNode := newChild$ \tcp*{this occurs only when the left and right children are merged and newNode has only one child}
    }
    \textbf{if} \textup{!}$\,root$.\textup{\texttt{CAS}}($curr, newNode$) \textbf{then} \textbf{return} \textup{\texttt{nullptr}}\;
    \label{alg15:line194}
}
\textbf{else if} \textup{!}$\,prev \rightarrow ptr[pidx]$.\texttt{CAS}($curr, newNode$) \textbf{then} \textbf{return} \textup{\texttt{nullptr}}\;
\label{alg15:line195}
\textbf{return} $newNode$\;
\end{algorithm}


==> algorithm/range_query.tex <==
\begin{algorithm}[H]
\label{range_query}
\caption{\texttt{rangeQuery}(low, high)}
vector<pair<key,value$>>$ $res$\;
int $ts :=$ \texttt{addTimestamp()}\;
\label{alg4:line83}
Node* $currNode := root$\;
\While{\textup{!}$\,currNode \rightarrow isLeaf$}
{
    Search $currNode$ for the appropriate child based on $key$\;
    Set $currNode$ to said child\;
}
Node* $prevNode :=$ \texttt{nullptr}\;
\While{$currNode \neq$ \textup{\texttt{nullptr}}}
{
\If{$currNode \rightarrow newNext \neq$ \textup{\texttt{nullptr}} $\&\& \ currNode \rightarrow newNext \rightarrow ts \leq ts$}
    {
        \label{alg5:line93}
        $currNode := currNode \rightarrow newNext$\;
        \label{alg5:line94}
        \textbf{if} $prevNode \neq$ \texttt{nullptr} \textbf{then} $prevNode \rightarrow next := currNode$\;
    }
    \Else
    {
        $res := list$.\texttt{rangeQuery}($low,\ high,\ ts,\ res$)\;
        $prevNode := currNode$,\ $currNode := currNode \rightarrow next$\;
        \textbf{if} $currNode \rightarrow list$'s first key $> high$ \textbf{then} \textbf{return} $res$\;
    }
}
\textbf{return} $res$\;
\end{algorithm}

==> algorithm/read.tex <==
\begin{algorithm}
\caption{\texttt{\textbf{Contains}} (key)}
\label{Read}
\footnotesize

$ix := models \rightarrow find\_idx(key)$\;
 \label{find_contains}
\uIf{$keys[ix] = key$}
{
    \texttt{\textbf{return}} vals[ix];
    \label{find_return}  
}
\Else{
    $current\_level\_bin :=  level\_bins[ix]$\;
    \If{$current\_level\_bin == null$}
    {
        \texttt{\textbf{return}} false
            \label{find_return_false}  
    }
    \ElseIf{$current\_level\_bin\rightarrow is\_node$}
    {
        \texttt{\textbf{return}} $current\_level\_bin \rightarrow child\_node \rightarrow Contains(key)$
    }
    \Else{
    \texttt{\textbf{return}} $current\_level\_bin \rightarrow child\_bin \rightarrow find(key)$
    }
}
\end{algorithm}


==> algorithm/search_tree.tex <==
\begin{algorithm}[H]
\label{searchtree}
\caption{\texttt{search}(key)}
Node* $currNode := root$\;
\While{\textup{!}$\,currNode \rightarrow isLeaf$}
{
    Search $currNode$ for the appropriate child based on $key$\;
    Set $currNode$ to said child\;
}
llNode* $foundNode := currNode \rightarrow list$.\texttt{llFind}($key$)\;
\If{$foundNode \rightarrow key = key$}
{
    \textbf{return} \texttt{read} $(foundNode)$\;
}
\Else
{
    \textbf{return} -1\;
}
\end{algorithm}

==> algorithm/set_help_idx.tex <==
\begin{figure}[H]
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\begin{multicols}{2}
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}\scriptsize
\algrestore{delete}
\Procedure{\textbf{\search}}{key}
\State{Node* $currNode := root$}
\While{\textup{!}$\,currNode \rightarrow isLeaf$}
    \State{Search $currNode$ for the appropriate child based on $key$}
    \State{Set $currNode$ to said child}
\EndWhile
\State{llNode* $foundNode := currNode \rightarrow$ \texttt{llFind}($key$)}
\If{$foundNode \rightarrow key = key$}
    \State{\textbf{return} \texttt{read} $(foundNode)$}
\Else
    \State{\textbf{return} \textup{"Key Not Found"}}
\EndIf
\EndProcedure
\algstore{search}
\end{algorithmic}
\hrule
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}\scriptsize
\algrestore{search}
% \State{\hrulefill}
\Procedure{\textbf{setHelpIdx}}{currIdx}   
\If{$helpIdx \neq -1$} {  \textbf{return} \texttt{false}}
\ElsIf{ \texttt{!}$helpIdx$\texttt{.CAS}$(-1,\ currIdx)$} 
\label{alg17:line218}
\State{  \textbf{return} \texttt{false}}
% \label{alg17:line218}
\Else{ \textbf{return} \texttt{true}}
\EndIf
\EndProcedure
\algstore{setidx}
\end{algorithmic}
\hrule
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}\scriptsize
\algrestore{setidx}
\Procedure{\textbf{\rangeQuery}}{low,high}
\State{vector $\langle$ pair $\langle$ key,value$\rangle \rangle$ $res$}
\State{int $ts :=$ \texttt{addTimestamp()}}
\label{alg4:line83}
\State{Node* $currNode := root$}
\While{\textup{!}$\,currNode \rightarrow isLeaf$}
% {
    \State{Search $currNode$ for the appropriate child based on $key$}
    \State{Set $currNode$ to said child}
% }
\EndWhile
\State{Node* $prevNode :=$ \texttt{nullptr}}
\While{$currNode \neq$ \textup{\texttt{nullptr}}}
{
\If{$currNode \rightarrow newNext \neq$ \textup{\texttt{nullptr}} $\&\& \ currNode \rightarrow newNext \rightarrow ts \leq ts$}
    % {
        \label{alg5:line93}
        \State{$currNode := currNode \rightarrow newNext$}
        \label{alg5:line94}
        \If {$prevNode \neq$ \texttt{nullptr}} {$prevNode \rightarrow next := currNode$}
        \EndIf
    % }
    \Else
    % {
        \State{$res := currNode$.\texttt{rangeQuery}($low, high, ts, res$)}
        \State{$prevNode := currNode$} \State{$currNode := currNode \rightarrow next$}
        \If{$currNode$'s first key $> high$} \State{\textbf{return} $res$}
        \EndIf
    % }
    \EndIf
}
\EndWhile
\State{\textbf{return} $res$}
% \\
% \hline
% \vspace{0.2pt}
\EndProcedure
\algstore{rangequery}
\end{algorithmic}
\end{multicols}
\caption{Pseudocode of \search, setHelpIdx and \rangeQuery}
\label{sethelpidx}
\end{figure}

==> algorithm/split_internal.tex <==
\begin{figure}[H]

% \renewcommand{\figurename}{Algorithm}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\begin{multicols}{2}

\end{multicols}
\end{figure}

==> algorithm/split_leaf.tex <==
\begin{algorithm}[H]
\label{splitleaf}
\caption{\texttt{splitLeaf}(prevNode,\ prevIdx,\ currNode,\ currIdx)}
$\textup{Node* } leftChild :=$ \texttt{new leafNode()}\;
$\textup{Node* } rightChild :=$ \texttt{new leafNode()}\;
$leftChild \rightarrow next := rightChild$ \; \label{alg19:line237}
$rightChild \rightarrow next := next$ \;
Split \textit{\textbf{this}} node into a pair of nodes pointed to by $leftChild$ and $rightChild$\;
\label{alg19:line233}
\If{\textup{!}$\ newNext$.\texttt{\textup{CAS}}($nullptr,\ leftChild$)}{
    \label{alg19:line234}
    $leftChild := newNext$\;
    $rightChild := leftChild \rightarrow next$\;
}

$\textup{Node* } newNode :=$ \texttt{new internalNode()}\;
Copy elements from $currNode$ to $newNode$ replacing $currChild$ with the two pointers $leftChild$ and $rightChild$\; \label{alg19:line239}
\If{$prevNode =$ \textup{\texttt{nullptr}}}
{
    \textbf{if} \textup{!}$\,root$.\texttt{CAS}($currNode,\ newNode$) \textbf{then} \textbf{return} \texttt{nullptr}\; \label{alg19:line241}
}
\textbf{else if} (!$\,prevNode \rightarrow ptr[prevIdx]$.\texttt{CAS}($currNode,\ newNode$) \textbf{then} \textbf{return} \texttt{nullptr}\; \label{alg19:line242}
\textbf{return} $newNode$\;
\end{algorithm}

==> algorithm/split_root_internal.tex <==
\begin{algorithm}[H]
\label{splitrootinternal}
\caption{\texttt{splitRootInternal}}
\texttt{markInternal()}\;
$\textup{Node* } leftChild :=$ \texttt{new internalNode()}\;
$\textup{Node* } rightChild :=$ \texttt{new internalNode()}\;
Split \textbf{\textit{this}} node into a pair of nodes pointed to by $leftChild$ and $rightChild$\;
$\textup{Node* } newNode :=$ \texttt{new internalNode()}\;
$newNode \rightarrow ptr[0] := leftChild$\;
$newNode \rightarrow ptr[1] := rightChild$\;
$newNode \rightarrow ptr[1] := $ first key from the second half of the current list of keys\;
\textbf{if} \textup{!}$\,root$.\texttt{CAS}($this,\ newNode$) \textbf{then} \textbf{return} \texttt{nullptr}\;
\textbf{return} $newNode$\;
\end{algorithm}

==> algorithm/split_root_leaf.tex <==
\begin{algorithm}[H]
\label{splitrootleaf}
\caption{\texttt{splitRootLeaf}}
$\textup{Node* } leftChild :=$ \texttt{new leafNode()}\;
$\textup{Node* } rightChild :=$ \texttt{new leafNode()}\;
$leftChild \rightarrow next := rightChild$ \;
$rightChild \rightarrow next := next$ \;
Split \textit{\textbf{this}} node into a pair of nodes pointed to by $leftChild$ and $rightChild$\;
\If{\textup{!}$\ newNext$.\texttt{\textup{CAS}}($nullptr,\ leftChild$)}{
    $leftChild := newNext$\;
    $rightChild := leftChild \rightarrow next$\;
}

$\textup{Node* } newNode :=$ \texttt{new internalNode()}\;
$newNode \rightarrow ptr[0] := leftChild$\;
$newNode \rightarrow ptr[1] := rightChild$\;
$newNode \rightarrow key[0] := rightChild's$  first key\;
\textbf{if} \textup{!}$\,root$.\texttt{CAS}($this,\ newNode$) \textbf{then} \textbf{return} \texttt{nullptr}\; 
\textbf{return} $newNode$\;
\end{algorithm}

==> algorithm/version_tracker/add_timestamp.tex <==
\begin{algorithm}[H]
\label{addtimestamp}
\caption{\texttt{addTimestamp}()}
\While{\textup{\texttt{true}}}{
    $currTail := tail$\;
    TrackerNode* $\ newTail :=$ \texttt{new TrackerNode}$(currTail \rightarrow ts + 1 ,\ sentinelLast)$\;
    \If{$currTail \rightarrow next$.\textup{\texttt{CAS}} $(sentinelLast,\ newTail)$}{
        $tail$.\texttt{CAS}$(currTail,\ newTail)$\;
        \textbf{return} $newTail \rightarrow ts$\;
    }
    \Else{
        \While{\textup{\texttt{true}}}{
            $currTail := tail$\;
            \textbf{if} $currTail \rightarrow next = sentinelLast$ \textbf{then return}\;
            \textbf{else} $tail$.\texttt{CAS}$(currTail,\ currTail \rightarrow next)$\;
        }
    }
}
\end{algorithm}

==> algorithm/version_tracker/get_latest_timestamp.tex <==
\begin{algorithm}[H]
\label{getlatestts}
\caption{int \texttt{getLatestTs}()}
\textbf{return} $tail \rightarrow ts$\;
\end{algorithm}

==> algorithm/version_tracker/remove_head.tex <==
\begin{figure}
% \begin{multicols}{2}
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{}
\scriptsize
\algrestore{wfllinsert}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\Procedure{\textbf{removeHead()}}{}
% \label{llfind}
\label{removehead}
% \caption{\texttt{removeHead}()}
\State{$currHead := head$}
\While{$currHead \rightarrow finish$}
    \State{$head$.\texttt{CAS}$(currHead,\ currHead \rightarrow next)$}
    \State{$currHead := head$}
% }
\EndWhile
\State{\textbf{return} $currHead$}
\EndProcedure
\algstore{removehead}
\end{algorithmic}
\hrule 

\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{}
\scriptsize
\algrestore{removehead}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\Procedure{\textbf{addTimestamp()}}{}
\While{\textup{\texttt{true}}}
    \State{$currTail := tail$}
    \State{TrackerNode* $\ newTail :=$ \texttt{new TrackerNode} $(currTail \rightarrow ts + 1 ,\ sentinelLast)$}
    \If{$currTail \rightarrow next$.\textup{\texttt{CAS}} $(sentinelLast,\ newTail)$}
        \State{$tail$.\texttt{CAS}$(currTail,\ newTail)$}
        \State{\textbf{return} $newTail \rightarrow ts$}
    
    \Else
        \While{\textup{\texttt{true}}}
            \State{$currTail := tail$}
            \If{$currTail \rightarrow next = sentinelLast$} \State{\textbf{return}}
            \Else
            \State{$tail$.\texttt{CAS}$(currTail,\ currTail \rightarrow next)$}
            \EndIf
        \EndWhile
    \EndIf

\EndWhile
\EndProcedure
\end{algorithmic}
% \end{multicols}
\caption{Pseudocode of removeHead and addTimestamp}
\label{alg:remHead}
\end{figure}

==> algorithm/wfdelete_leaf.tex <==
\begin{algorithm}[H]
\label{wfdeletefromleaf}
\caption{\texttt{wfDeleteFromLeaf}(key,\ tid,\  phase)}
\textbf{if} $frozen$ \textbf{then} \textbf{return} \texttt{false}\;
$currState := stateArray[tid]$\;
$currNode := currState \rightarrow searchNode$\;
\label{alg10:line136}
\If{$currNode == nullptr$}{
    $currState \rightarrow finished := true $\;
    \textbf{return} \texttt{true}\;
}
\If{$currNode == dummyNode$}{
    $node := list$.\texttt{llFind}$(key)$\;
    \label{alg11:find}
    $currState \rightarrow searchNode.$\texttt{CAS}$(dummyNode, Node)$\;
    \label{alg10:line142}
}
$\textup{llNode*} \ node := currState \rightarrow searchNode$\;
\If{$node == nullptr$}{
    $currState \rightarrow finished := true $\;
    \textbf{return} \texttt{true}\;
}
\uIf{$node \rightarrow key == key$}
{
    \texttt{bool} $res := list$.\texttt{wfLLInsert}($key$, -1,\ tid,\ phase)\;
    \label{alg10:line151}
    \If{res}{$currState \rightarrow finished := true$\;}
    \textbf{return} \texttt{res}\;
}
\Else{
    $currState \rightarrow finished := true$\;
    \textbf{return} \texttt{true}\;
}
\end{algorithm}


==> algorithm/wfinsert_leaf.tex <==
\begin{figure}
\begin{multicols}{2}
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{}
\scriptsize
\algrestore{borrowhelper}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\Procedure{\textbf{wfInsertLeaf}}{key,\ value,\ tid,\ ph}
% \label{wfinsertintoleaf}
% \caption{\texttt{wfInsertIntoLeaf}(key,\ value,\ tid,\ phase)}
\If{$frozen$}
\State{\textbf{return} \texttt{"Failed"}}
\EndIf
\If{$count \geq MAX$}
% {
    \State{\texttt{freezeLeaf()}}
    \State{\textbf{return} \texttt{"Failed"}}
% }
\Else 
\State{res := \texttt{\textup{wfLLInsert}}($key,\ value,\ tid,\ ph$)}
\If{res = \texttt{"New Key Inserted"}}
    \State{$count$++}
\EndIf
\textbf{return} \texttt{res}
\EndIf
\EndProcedure
\algstore{wfllinsert}
\end{algorithmic}
\hrule
\begin{algorithmic}[1]
\renewcommand{\algorithmicprocedure}{}
% \label{}
\scriptsize
\algrestore{wfllinsert}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}
\Procedure{\textbf{wfDeleteLeaf}}{key,\ tid,\ phase}
% \caption{\texttt{wfDeleteFromLeaf}(key,\ tid,\  phase)}
\State{$currState := stateArray[tid]$}
\State{$currNode := currState \rightarrow searchNode$}
\label{alg10:line136}
\If{$currNode = nullptr$}
    \State{$currState \rightarrow finished := true $}
    \State{\textbf{return} \texttt{"Operation Finished"}}
\EndIf
\If{$currNode = dummyNode$}
    \State{$node := list$.\texttt{find}$(key)$}
    \label{alg11:find}
    \State{$currState \rightarrow searchNode.$\texttt{CAS} $(dummyNode, Node)$}
    \label{alg10:line142}
\EndIf
\State{$\textup{llNode*} \ node := currState \rightarrow searchNode$}
\If{$node == nullptr$}
    \State{$currState \rightarrow finished := true $}
    \State{\textbf{return} \texttt{"Operation Finished"}}
\EndIf
\If{$node \rightarrow key = key$}
% {
    \State{\texttt{wfLLInsert}($key$, -1,\ tid,\ phase)}
    \label{alg10:line151}
    \State{$currState \rightarrow finished := true$}
    \State{\textbf{return} \texttt{"Operation Finished"}}
% }
\Else
    \State{$currState \rightarrow finished := true$}
    \State{\textbf{return} \texttt{"Operation Finished"}}
\EndIf
\EndProcedure
\algstore{wfdeleteleaf}
\end{algorithmic}
\end{multicols}
\caption{Pseudocode of wfInsertLeaf snd wfDeleteLeaf \op}
\end{figure}

==> figs/OpenBwTree_vs_Uruv.tex <==
\begin{center}
\begin{tabular}{ccc}
    \multicolumn{3}{c}{\includegraphics[width = 0.7\linewidth]{image/legend_URUV1.png}}\\   
     \includegraphics[width=0.33\linewidth]{image/100read.pdf} &
     \includegraphics[width=0.33\linewidth]{image/ReadHeavy.pdf} &
     \includegraphics[width=0.33\linewidth]{image/UpdateHeavy.pdf}
     \\
     (a) & (b) & (c) \\
\end{tabular}
\scriptsize
\captionof{figure}{\scriptsize The performance of \textbf{Uruv} when compared to \textbf{LF$\_$B+Tree}\cite{braginsky+:SPAA:2012} and \textbf{Open$\_$BwTree}\cite{wang2018building}. Higher is better. The workload distributions are (a) Reads - 100\% (b) Reads - 95\%, Updates - 5\%, and (c) Reads - 50\%, Updates - 50\%}
\label{fig:uruv-anastasia-openbwtree}
\end{center}
% \label{fig:uruv-anastasia-openbwtree}
% \begin{figure*}[ht]
% % \captionsetup[subfigure]{justification=centering}
% \centering
% \begin{subfigure}{}
%   \includegraphics[width=0.31\linewidth]{image/Read 100 Anastasia vs OpenBw tree vs URUV.pdf}
%   \subcaption{a}
% \end{subfigure}
% \begin{subfigure}{}
%   \includegraphics[width=0.31\linewidth]{image/Read 95 Anastasia vs OpenBw tree vs URUV.pdf}
% \end{subfigure}
% \begin{subfigure}{}
%   \includegraphics[width=0.31\linewidth]{image/Read 50 Anastasia vs OpenBw tree vs URUV.pdf}
% \end{subfigure}
% \caption{The performance of \textbf{Uruv} when compared to \textbf{LFB$^+$Tree} and \textbf{OpenBw-Tree}. Higher is better. The workload distributions are (a) Reads - 100\% (b) Reads - 95\%, Updates - 5\%, and (c) Reads - 50\%, Updates - 50\%}
% \label{fig:uruv-anastasia-openbwtree}
% \end{figure*}

==> figs/VCAS_BST_vs_Uruv.tex <==
\begin{tabular}{ccc}
    \multicolumn{3}{c}{\includegraphics[width=0.7\linewidth]{image/UruvLegend2.png}}\\
   \includegraphics[width=0.32\linewidth]{image/94read.pdf}  & 
   \includegraphics[width=0.32\linewidth]{image/90read.pdf} & 
   \includegraphics[width=0.32\linewidth]{image/85read.pdf} \\
   (a) & (b) & (c) \\
   \includegraphics[width=0.32\linewidth]{image/49read.pdf} &
   \includegraphics[width=0.32\linewidth]{image/45read.pdf} &
   \includegraphics[width=0.32\linewidth]{image/40read.pdf} \\
   (d) & (e) & (f)
\end{tabular}
\captionof{figure}{\scriptsize The performance of \textbf{Uruv} when compared to \textbf{VCAS-BST}. The workload distributions are (a) Reads - 94\%, Updates - 5\%, Range Queries of size 1K - 1\%, (b) Reads - 90\%, Updates - 5\%, Range Queries of size 1K - 5\%, (c) Reads - 85\%, Updates - 5\%, Range Queries of size 1K - 10\%, (d) Reads - 49\%, Updates - 50\%, Range Queries of size 1K - 1\%, (e) Reads - 45\%, Updates - 50\%, Range Queries of size 1K - 5\%, and (f) Reads - 40\%, Updates - 50\%, Range Queries of size 1K - 10\%}
\label{fig:5d-5f}
% \begin{figure*}[ht]
% \captionsetup[subfigure]{justification=centering}
% \centering
% \subfloat[]{%
%   \includegraphics[width=0.32\linewidth]{image/Read 94 VCAS BST vs URUV.pdf}%
% }
% \subfloat[]{%
%   \includegraphics[width=0.32\linewidth]{image/Read 90 VCAS BST vs URUV.pdf}%
% }
% \subfloat[]{%
%   \includegraphics[width=0.32\linewidth]{image/Read 85 VCAS BST vs URUV.pdf}%
% }
% \vspace{1em}
% \subfloat[]{%
%   \includegraphics[width=0.32\linewidth]{image/Read 49 VCAS BST vs URUV.pdf}%
% }
% \subfloat[]{%
%   \includegraphics[width=0.32\linewidth]{image/Read 45 VCAS BST vs URUV.pdf}%
% }
% \subfloat[]{%
%   \includegraphics[width=0.32\linewidth]{image/Read 40 VCAS BST vs URUV.pdf}%
% }
% \caption{The performance of \textbf{Uruv} when compared to \textbf{VCAS-BST}. The workload distributions are (a) Reads - 94\%, Updates - 5\%, Range Queries of size 1K - 1\%, (b) Reads - 90\%, Updates - 5\%, Range Queries of size 1K - 5\%, (c) Reads - 85\%, Updates - 5\%, Range Queries of size 1K - 10\%, (d) Reads - 40\%, Updates - 50\%, Range Queries of size 1K - 1\%, (e) Reads - 45\%, Updates - 50\%, Range Queries of size 1K - 5\%, and (f) Reads - 40\%, Updates - 50\%, Range Queries of size 1K - 10\%}
% \label{fig:5d-5f}
% \end{figure*}

==> figs/WFstructure.tex <==
% \begin{figure}[h]

    \centering
    \begin{minipage}[t]{.53\textwidth}
    \begin{lstlisting}[backgroundcolor=\color{white}, basicstyle=\scriptsize]
State* stateArray[totalThreads]

class HelpRecord{     
    long currTid; 
    long lastPhase;
    long nextCheck;
}
    \end{lstlisting}
    \end{minipage}
     \begin{minipage}[t]{.46\textwidth}
    \begin{lstlisting}[backgroundcolor=\color{white}, basicstyle=\scriptsize]
  class State{           
      long phase;
      bool finished;
      Vnode* vnode;
      long key;
      long value; 
      llNode* searchNode
  }

    \end{lstlisting}
    \end{minipage}
% \end{mdframed}
% \caption{Tree  Data Structure}
% \end{figure}


==> figs/main_algo_fig.tex <==
\begin{figure}
\begin{minipage}{.32\linewidth}
% \vspace{3em}
    \centering
    \includegraphics[width = 1 \linewidth]{image/split.pdf}
    \textbf{(a)}
\end{minipage}
\begin{minipage}{.32\linewidth}
    \centering
    \includegraphics[width = 1 \linewidth]{image/merge.pdf}
    \textbf{(b)}
\end{minipage}
\begin{minipage}{.32\linewidth}
      \centering
      \includegraphics[width = 1 \linewidth]{image/Split_Internal.pdf}
    \textbf{(c)}
\end{minipage}
\caption{(a) Split Leaf, (b) Merge Leaf, (c) Split Internal}
\label{fig:Tree Operations}
\end{figure}



==> figs/tree_class.tex <==
\begin{minipage}[t]{0.32\linewidth}
\begin{lstlisting}[basicstyle=\scriptsize]
Uruv{              
    Node* root;           
}
InternalNode: Node{
    long key[MAX]
    Node* ptr[MAX+1]
    helpidx
}
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.32\linewidth}
\begin{lstlisting}[basicstyle=\scriptsize]

LeafNode: Node{
    VLF_LL* ver_head;
    LeafNode* next;
    LeafNode* newNext;
    int ts
}
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.32\linewidth}
\begin{lstlisting}[basicstyle=\scriptsize]

Node{           
    long count;
    bool isLeaf;
    bool frozen;
}
\end{lstlisting}
\end{minipage}

==> figs/version_tracker.tex <==
\begin{figure}[!thb]	
	\begin{multicols}{2}
 \scriptsize
 % \begin{multicols}{2}
\begin{lstlisting}
class TrackerNode{
    int ts;
    atomic<TrackerNode*> next;
    bool finished;
}
\end{lstlisting}
\begin{lstlisting}
class TrackerList{
    TrackerNode* head;
    TrackerNode* tail;
    TrackerNode* sentinelLast;
}
\end{lstlisting}
\end{multicols}
\caption{Version Tracker Data Structure}
\label{fig:version_tracker}
\end{figure}


% \begin{mdframed}
%     \centering
%     \begin{minipage}[t]{.53\textwidth}
%     \begin{lstlisting}[backgroundcolor=\color{white}]
% class TrackerNode{
%     int ts;
%     atomic<TrackerNode*> next;
%     bool finished;
% }
%     \end{lstlisting}
%     \end{minipage}
%     \vrule
%      \begin{minipage}[t]{.46\textwidth}
%     \begin{lstlisting}[backgroundcolor=\color{white}]
% class TrackerList{
%     TrackerNode* head;
%     TrackerNode* tail;
%     TrackerNode* sentinelLast;
% }
%     \end{lstlisting}
%     \end{minipage}
% \end{mdframed}

==> figs/vl_fll.tex <==

\begin{figure}[h]
    \centering
    % \begin{mdframed}
    \begin{minipage}[t]{0.32\linewidth}
    % \begin{subfigure}{.32\textwidth}
    \begin{lstlisting}[basicstyle=\scriptsize]
Vnode{
    value_t value;
    int ts;
    Vnode* nextv;
}
    \end{lstlisting}
    \end{minipage}
    % \end{subfigure}
    % \vrule
    \begin{minipage}[t]{0.32\linewidth}
    \begin{lstlisting}[basicstyle=\scriptsize]
llNode{
      key_t key;
      Vnode* vhead;
      llNode* next;
}
    \end{lstlisting}
    \end{minipage}
    % \vrule
     \begin{minipage}[t]{0.32\linewidth}
    \begin{lstlisting}[basicstyle=\scriptsize]
VLF_LL{

      llNode* head;
    
}
    \end{lstlisting}
    \end{minipage}
    % \end{mdframed}
\caption{Versioned Lock-Free Linked-List Data Structure}
\label{fig:vlfll}
\end{figure}


==> listing/model.tex <==
\mdfdefinestyle{MyFrame}{%
    linecolor=black,
    outerlinewidth=2pt,
    %roundcorner=20pt,
    innertopmargin=1.5pt,
    innerbottommargin=0pt,
    innerrightmargin=4pt,
    innerleftmargin=4pt,
        leftmargin = 4pt,
        rightmargin = 4pt
    %backgroundcolor=gray!50!white}
        }

% \begin{mdframed}
% \centering
\begin{figure}
\begin{lstlisting}

class Bin{
        Node* child_node;
        Child_Bin* child_bin;
        Bool is_node;
}

class Node{
    LinearModel models[];
    key_type keys[];
    val_type vals[];
    atomic<Bin*> level_bin[];
}
\end{lstlisting}
\caption{Kanva Model Design Structure}
\label{fig::Model}
\end{figure}
% \end{mdframed}

==> table/time.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\caption{Time taken for building the structure}
\label{time}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|l|}{Workloads}                         & books   & fb  & osmc & normal & log normal & uniform\_sparse \\ \hline
\multicolumn{2}{|l|}{Number of Data} & 200M    & 200M    & 200M  & 200M  & 200M    & 200M  \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{Time}} & LPA & 92.1056 & 105 & 98.9 & 100.9  & 117.1      & 83.7            \\ \cline{2-8} 
\multicolumn{1}{|l|}{}   & PGM       & 41.4    & 56      & 53.2  & 64.4  & 64.4    & 38.4  \\ \cline{2-8} 
\multicolumn{1}{|l|}{}   & (a,b)-tree   & 278.4   & 277.2   & 273.9 & 273.2 & 278.3   & 274.7 \\ \cline{2-8} 
\multicolumn{1}{|l|}{}   & C-IST      & 45406.4 & 42532.9 &  48895.5     &  46243.1     & 45751.1 &   48215.1    \\ \hline
\end{tabular}%
}
\end{table}
